Higgs boson couplings: measurements and theoretical interpretation

This report will review the Higgs boson properties: the mass, the total width and the couplings to fermions and bosons. The measurements have been performed with the data collected in 2011 and 2012 at the LHC accelerator at CERN by the ATLAS and CMS experiments. Theoretical frameworks to search for new physics are also introduced and discussed.

==> HCS1.tex <==

%\section{Higgs boson phenomenology: production and decay}
%\label{sec:Theory}

This Section is not intended to provide a complete phenomenological profile of the Higgs boson
but only to recap few essential informations that are needed to understand the experimental
results and their theoretical interpretations.

At LHC the production of the Standard Model (SM) Higgs boson occurs via the following processes, 
listed in order of decreasing cross section at $7{-}8\UTeV$ center-of-mass energy in
Tab.~\ref{Pxs}.
%---
\begin{table}[hbt]
\tbl{$\PH$ production cross sections.}
{\begin{tabular}{@{}lll@{}} \toprule
 & & \\ \colrule
gluon fusion production        & $\Pg\Pg\to \PH$            & Fig.~\ref{fig:feyn_ggF} \\
vector boson fusion production & $\PQq\PQq \to \PQq\PQq\PH$ & Fig.~\ref{fig:feyn_VBF} \\
associated production with a $\PW$ boson & $\PQq\PQq \to \PW\PH$ & Fig.~\ref{fig:feyn_vH} \\ 
or with a $\PZ$ boson                    & $\Pp\Pp \to \PZ\PH$ & Figs.~\ref{fig:feyn_vH}, 
\ref{fig:feyn_ggZH2} and~\ref{fig:feyn_ggZH1} \\
including a small~($\sim 8\%$) but less precisely known contribution from & $\Pg\Pg \to \PZ\PH$
& \\ 
associated production with a pair of top or bottom quarks & $\PQq\PQq, \Pg\Pg \to \PAQt\PQt\PH$ 
or $\to \PAQb\PQb\PH$ & Fig.~\ref{fig:feyn_ttH} \\
associated production with a single top quark & $\PQq\Pg \to \PQt\PH$ & Fig.~\ref{fig:feyn_tH} \\ 
\botrule
\end{tabular} \label{Pxs}}
\end{table}
%--
\begin{figure}[hbt]
\begin{center}
% \input {Figures/feyn_ggF.tex}
    \label{fig:feyn_ggF}
    \hspace*{2.0cm}
 %   \input {Figures/feyn_VBF.tex}
    \label{fig:feyn_VBF}
 \end{center}
\caption[]{Examples of leading-order Feynman diagrams for Higgs boson production via 
the (a) $\Pg\Pg\to \PH$  and (b) $\PQq\PQq \to \PQq\PQq\PH$ production processes.}
\label{fig:feyn_ggFVBF}
\end{figure}
%--
\begin{figure}[hbt]
\begin{center}
%\input {Figures/feyn_Vh.tex}
    \label{fig:feyn_vH}
    \hspace{0.5cm}
%\input {Figures/feyn_ggZH2.tex}
    \label{fig:feyn_ggZH2}
    \hspace{0.5cm}
%\input {Figures/feyn_ggZH1.tex}
    \label{fig:feyn_ggZH1}
    \hspace{0.5cm}
\end{center}
  \caption[]{Examples of leading-order Feynman diagrams for Higgs boson production via the (a) 
$\PQq\PQq \to \PV\PH$ and (b,~c)~$\Pg\Pg \to \PZ\PH$ production processes.}
\label{fig:feyn_prod}
\end{figure}
%--
\begin{figure}[hbt]
\begin{center}
 %   \input {Figures/feyn_tth3.tex}
    \hspace{0.5cm}
 %\input {Figures/feyn_tth1.tex}
    \hspace{0.5cm}
  %\input {Figures/feyn_tth2.tex}
    \hspace{0.5cm}
\end{center}
\caption[]{Examples of leading-order Feynman diagrams for Higgs boson production in 
association with $\PAQt\PQt$ or $\PAQb\PQb$}
\label{fig:feyn_ttH}
\end{figure}
%--
\begin{figure}[hbt]
\begin{center}
 %\input {Figures/feyn_tH1_alt.tex}
    \label{fig:feyn_tHjb1}
%\input {Figures/feyn_tH2_alt.tex}
    \hspace{0.5cm}
    \label{fig:feyn_tHjb2}
%\input {Figures/feyn_tH3_alt.tex}
    \label{fig:feyn_WtH1}
%\input {Figures/feyn_tH4.tex}
    \label{fig:feyn_WtH2}
\end{center}
\caption[]{Examples of leading-order Feynman diagrams for Higgs boson production in 
association with a single top quark. }  
\label{fig:feyn_tH}
\end{figure}
%--
% CM some additions in CAPITAL LETTER - to check 
The HIGGS BOSON $\PH$ field is the custodial singlet in THE GROUP  $\lpar 2_{\ssL}\,\otimes\,2_{\ssR}\rpar = 
1\,\oplus\,3$ contained in a scalar doublet $\upPhi$ of hypercharge $1/2$. THE FIELD $\Upphi$ develops 
a vacuum expectation value (VEV) and $\PH$ is the quantum fluctuation around the VEV. This has 
the consequence that the fermion masses and the Yukawa couplings are not independent quantities, \ie 
$\PH$ couples to a fermion-anti-fermion pair of the same flavour, with a coupling proportional 
to the mass of the fermion. Equivalently, $\PH$ couples to vector boson ($\PW\PW$ or $\PZ\PZ$) 
proportionally to their mass. This simple fact will have deep consequences when trying to build 
a model independent framework for SM deviations.

In order to make the results of this Section transparent we stress the conceptual separation
between diagrams, amplitudes and (pseudo-)observables. 

Diagrams, made of propagators and vertices, describe the couplings and the propagation and, in 
general, are not separately gauge invariant. 

(Sub-)Amplitudes collect set of diagrams, \eg the resonant (often called ``signal'') and the 
non-resonant (often called ``background'') part of a physical process (which may contain more 
than one resonant part) and, once again, they are not separately gauge invariant. 

Finally, (pseudo-)observables are elements (or are related to elements) of the $\mrS\,$-matrix, 
\eg partial decay widths or production cross sections. Therefore, for a light Higgs boson it 
makes sense to talk about $\PH \to \PV\PV$ or $\PH \to \PAf\Pf$ couplings, but objects like partial 
decay widths, \eg  $\Gamma_{\PH \to \PV\PV}$, (forbidden by kinematics) can only be given and 
interpreted within a certain set of conventions. Actually, it is not only a question of 
kinematics, $\PH$ and $\PW\,,\,\PZ$ are unstable particles whose theoretical  treatment is far 
from trivial and presents a certain number of subtleties~\cite{Passarino:2010qk,Goria:2011wa}.
%--
% CM changed the order. Shall we keep the "remark" in bold ?
%CM It is ZWA or Narrow WA ?
Finally, a SM Higgs boson has a very narrow width, which means that theoretical, ``at the peak'',
predictions are provided in the so-called ``zero-width-approximation'' (ZWA), equivalent to
(on-shell) production cross section $\,\times\,$ (on-shell) decay.
%--
\begin{remark}
In essence, the whole game in determining the Higgs couplings has to do with extracting
vertices from (pseudo-)observables.
\end{remark}

Having that in mind, the results presented below have been obtained as 
follows~\cite{Dittmaier:2011ti,Dittmaier:2012vm,Heinemeyer:2013tqa}. The Higgs total width 
resulting from {\tt{HDECAY}}~\cite{Djouadi:1997yw} has been modified according to the prescription:
%--
\bq
\Gamma_{\PH} = \Gamma^{\mathrm{HD}} - \sum_{\PV=\PW, \PZ}\,\Gamma^{\mathrm{HD}}_{\PV} +
\Gamma^{\mathrm{Pr}}_{4\Pf} \spc
\eq
%--
where $\Gamma_{\PH}$ is the total Higgs width, $\Gamma^{\mathrm{HD}}$ the Higgs width obtained 
from {\tt{HDECAY}}, $\Gamma^{\mathrm{HD}}_{\PV}$ stands for the partial widths to $\PZ\PZ$ and 
$\PW\PW$ calculated with {\tt{HDECAY}}, while $\Gamma^{\mathrm{Pr}}_{4\Pf}$ represents the partial
width of $\PH \to 4\,\Pf$ calculated with {\tt{PROPHECY4F}}~\cite{Bredenstein:2007ec}. The latter 
can be split into the decays into $\PZ\PZ$, $\PW\PW$, and the interference,
%--
\bq
\Gamma^{\mathrm{Pr}}_{4\Pf} = \Gamma_{\PH \to \PW^*\PW^* \to 4\,\Pf} +
\Gamma_{\PH \to \PZ^*\PZ^* \to 4\,\Pf} +
\Gamma_{\PW\PW/\PZ\PZ-\mathrm{intf}} \spp
\eq
%--
Whenever $\PV^*$ appears it should be understood as follows: {\tt{PROPHECY4F}} calculations are
consistently performed with off-shell gauge bosons and it is valid above, near and below the 
gauge boson pair thresholds. For instance the definition is such that
%--
\bq
\Gamma_{\PH \to \PW^*\PW^* \to 4\,\Pf} = 
 9\,\Gamma_{\PH \to \PGne\Pep\PGm\PAGnGm} +
12\,\Gamma_{\PH \to \PGne\Pep\PQd\PAQu} +
 4\,\Gamma_{\PH \to \PQu\PAQd\PQs\PAQc} \spp
\eq
%--
These conventions are essential in understanding every statement of the form
``the $\PH$ decays to $\PW$ and $\PZ$ bosons \dots''.

%CM add the PO definition.
A complete generalization is represented by the LHC-PO (where PO stays for pseudo-observables)
framework~\cite{Gonzalez-Alonso:2015bha,Greljo:2015sla,Bordone:2015nqa,David:2015waa}; the idea 
of PO has been 
formalised the first time in the context of electroweak observables around the $\PZ$ pole at the LEP time REF?.
% CM add a reference ? which one, the experimental summary and some TH work?
On a more theoretical footing, the LHC POs are defined from a general decomposition of
on-shell amplitudes involving the Higgs boson and based on analyticity, unitarity, and crossing
symmetry and a momentum expansion.
%CM could you explain more the sentence above ?

Another useful definition concerns the ``leading order'': technically speaking leading-order (LO)
defines the order in perturbation theory where the process starts. Notice that sometimes ``LO''
is used to denote tree level (as opposite to loops).

Examples of LO Feynman diagrams for the Higgs boson decays are shown in 
Figs.~\ref{fig:feyn_hVVff} and~\ref{fig:feyn_hgg}. The decays to $\PW$ and $\PZ$ bosons 
(see Fig.~\ref{fig:feyn_hVV}) and to fermions (see Fig.~\ref{fig:feyn_hff}) start at tree level 
whereas the $\PH \to \PGg\PGg$ decay starts at one loop, being generated by loops containing 
heavy quark or bosons, see Fig.~\ref{fig:feyn_hgg}.
%--
\begin{figure}[hbt]
\begin{center}
 %\input {Figures/feyn_hVV.tex}
    \hspace{0.5cm}
    \label{fig:feyn_hVV}
%\input {Figures/feyn_hff.tex}
    \hspace{0.5cm}
    \label{fig:feyn_hff}
\end{center}
\caption[]{Examples of leading-order Feynman diagrams for Higgs boson decays (a) 
to $\PW$ and $\PZ$ bosons and (b) to fermions.}
\label{fig:feyn_hVVff}
\end{figure}

\begin{figure}[hbt!]
\begin{center}
  %  \input {Figures/feyn_hggf.tex}
    \hspace{0.5cm}
    %\input {Figures/feyn_hggW1.tex}
    \hspace{0.5cm}
    %\input {Figures/feyn_hggW2.tex}
    \hspace{0.5cm}
\end{center}
\caption[]{Examples of leading-order Feynman diagrams for Higgs boson decays to a pair of photons.}
  \label{fig:feyn_hgg}
\end{figure}
%--
The SM Higgs boson production cross sections and decay branching fractions have been calculated 
in the recents years at high order in perturbation theory.
The many calculations have been compared and then eventually combined and summarised in 
\Brefs{Dittmaier:2011ti,Dittmaier:2012vm,Heinemeyer:2013tqa}, and they are shown in 
Figs.~\ref{fig:figures_yr}. 
Following these calculations, additional and important progresses have been made, and many more calculations have been performed
at higher order, but they will not be reported here, since they have not been used in the analysis of the Run~1 data.
%--
%and are based on the extensive theoretical work documented 
%n Refs.~\cite{Georgi:1977gs,Djouadi:1991tka,Dawson:1990zj,Spira:1995rr,Harlander:2002wh,Anastasiou:2002yz,Ravindran:2003um,Catani:2003zt,Actis:2008ug,Anastasiou:2008tj,deFlorian:2009hc,deFlorian:2012yg,Bozzi:2005wk,deFlorian:2011xf,Grazzini:2013mca,Stewart:2011cf,Banfi:2012jm,Djouadi:1997yw,Bredenstein:2006rh,Bredenstein:2006ha,Denner:2011mq,Cahn:1983ip,Ciccolini:2007jr,Ciccolini:2007ec,Bolzoni:2010xr,Botje:2011sn,Lai:2010vv,Martin:2009iq,Ball:2010de,Glashow:1978ab,Brein:2003wg,Denner:2011id,Englert:2013vua,Ferrera:2014lca,Raitio:1978pt,Beenakker:2002nc,Dawson:2003zu,Harlander:2003ai,Dittmaier:2003ej,Dawson:2003kb,Harlander:2011aa,Farina:2012xp,Zeppenfeld:2000td,Duhrssen:2004cv}. 
%--
\begin{figure}[hbt]
\centering
\includegraphics[width=0.48\textwidth]{Figures/xs_yr.pdf}
\includegraphics[width=0.48\textwidth]{Figures/br_yr.pdf}
\caption[]{Standard Model Higgs production cross sections and Branching Ratios at $8\UTeV$ 
center of mass energy }
\label{fig:figures_yr}
\end{figure}
%--
After the LHC Run~1, the SM of particle physics has been completed, raising its status to that 
of a full theory. In particular, once the mass of the Higgs boson has been measured, all its properties 
have been fixed. 
%--
%\begin{example}[Results]
The inclusive cross sections and branching fractions for the most important 
production and decay modes are summarised with their overall uncertainties in 
Tabs.~\ref{tab:SMCrossSections} and~\ref{tab:SMBranchingFractions} for a Higgs boson 
mass of $125.09\UGeV$. The value of the mass being the one measured by the ATLAS and CMS 
collaboration with the Run~1 statistics.
%\end{example}
%--
\begin{table}[htbp]
\caption[]{Standard Model predictions for the Higgs boson production cross sections together 
with their theoretical uncertainties as of the year 2013. 
The value of the Higgs boson mass is  $m_{\PH}=125.09\UGeV$ as measured by the ATLAS and CMS experiments, 
and the predictions  are from \Bref{Heinemeyer:2013tqa}.
The $\Pp\Pp \to \PZ\PH$~cross section, calculated at NNLO in QCD, includes  both the 
quark-initiated, \ie $\PQq\PQq \to \PZ\PH$ or~$\PQq\Pg \to \PZ\PH$, and the 
$\Pg\Pg\to \PZ\PH$ contributions.  
The uncertainties in the cross sections are evaluated as the sum in quadrature of the 
uncertainties resulting from variations of the QCD scales, parton distribution functions, and 
$\alpha_{\text s}$. 
The uncertainty in the $\PQt\PH$ cross section is calculated following the procedure of 
\Bref{Alwall:2014hca}. 
The order of the theoretical calculations for the different production processes is also 
indicated in the table. In the case of $\PAQb\PQb\PH$~production, the values are given for the mixture of 
five-flavour~(5FS) and four-flavour~(4FS) schemes as recommended in~\Bref{Harlander:2011aa}.
}
\vspace*{-0.2cm}
%--
\begin{center}
\begin{tabular}{clr@{\hskip 0.4ex}lr@{\hskip 0.4ex}lc} \hline\hline
 &  \multicolumn{1}{c}{Production }  & \multicolumn{4}{c}{Cross section [pb]} & Order of  \\ \cline{3-6}
 &  \multicolumn{1}{c}{process}     &   \multicolumn{2}{c}{$\sqrt{s}=7$ TeV}   &  \multicolumn{2}{c}{$\sqrt{s}=8$ TeV} & calculation  \\ \hline
 &  ggF       &   $15.0$&${} \pm 1.6$      &  $19.2$&${}\pm 2.0$    & {\small\sc NNLO(QCD) + NLO(EW) } \\
 &  VBF       &   $1.22$&${}\pm 0.03$     &  $1.58$&${}\pm 0.04$   & {\small\sc NLO(QCD+EW) + approx.~NNLO(QCD) } \\
 &  WH        &   $0.577$&${}\pm 0.016$   &  $0.703$&${}\pm 0.018$ & {\small\sc NNLO(QCD) + NLO(EW) }  \\
 &  ZH        &   $0.334$&${}\pm 0.013$   &  $0.414$&${}\pm 0.016$ & {\small\sc NNLO(QCD) + NLO(EW) }  \\ 
 & ggZH       &   $0.023$&${}\pm 0.007$    &   $0.032$&${}\pm 0.010$      & {\small\sc NLO(QCD) } \\
 &  ttH       &   $0.086$&${}\pm 0.009$   &  $0.129$&${}\pm 0.014$ & {\small\sc NLO(QCD) } \\ 
 &  tH        &   $0.012$&${}\pm 0.001$   &  $0.018$&${}\pm 0.001$ & {\small\sc NLO(QCD) }   \\ 
 &  bbH       &   $0.156$&${}\pm 0.021$   &  $0.203$&${}\pm 0.028$ & {\small\sc 5FS NNLO(QCD) + 4FS NLO(QCD) }  \\ \hline
 &  Total       &   $17.4 $&${}\pm 1.6$     &  $22.3$&${}\pm 2.0$    &  \\
\hline\hline
\end{tabular}
\end{center}
\label{tab:SMCrossSections}
\end{table}
%--
\begin{table}[htbp]
\caption[]{Standard Model predictions for the decay branching fractions of a Higgs boson with 
a mass of $125.09\UGeV$ ~\cite{REF MASS}, together with their uncertainties~\cite{Heinemeyer:2013tqa}. }
\begin{center}
\begin{tabular}{clcr@{\hskip 0.4ex}l}\hline\hline
 &    Decay mode &\multicolumn{3}{c}{Branching fraction [\%]}  \\  \hline
 &     $Hbb$       & &   $57.5$&${}\pm 1.9$    \\
 &     $HWW$       & &   $21.6$&${}\pm 0.9$   \\
 &     $Hgg$       & &   $8.56$&${}\pm 0.86$  \\
 &     $Htt$       & &   $6.30$&${}\pm 0.36$  \\
 &     $Hcc$       & &   $2.90$&${}\pm 0.35$  \\
 &     $HZZ$       & &   $2.67$&${}\pm 0.11$  \\
 &     $H\gamma\gamma$       & &   $0.228$&${}\pm 0.011$  \\
 &     $HZ\gamma$       & &   $0.155$&${}\pm 0.014$  \\
 &     $H\mu\mu$       & &   ~~$0.022$&${}\pm 0.001$  \\ 
\hline\hline
\end{tabular} 
\end{center}
\label{tab:SMBranchingFractions}
\end{table} 

%--
\clearpage
%--

    
%--
 


==> HC_proleg.tex <==
\usepackage[dvipsnames]{xcolor}
%---
%\usepackage{axodraw}
\usepackage{graphicx}
\usepackage{amssymb}
%\usepackage{feynmp-auto}
\RequirePackage{mathptmx}
\RequirePackage[T1]{fontenc}
%---
\usepackage{heppennames2}
\usepackage{lhchiggs}
\usepackage{cernunits}
%---
% \usepackage{draftwatermark}
%---
%\usepackage[left]{lineno}
%\linenumbers
%---
\DeclareSymbolFont{forjmath}{OT1}{cmr}{m}{sl}
\DeclareMathSymbol{\Jmath}{\mathord}{forjmath}{'021}
\def\jmath{\Jmath}
\DeclareFontFamily{OT1}{cmr}{}
\DeclareFontFamily{OT1}{cmss}{}
%--
%\usepackage{pifont}
%\usepackage{colortbl}
%\usepackage{fancybox}
%\usepackage{ctable}
%\usepackage[center,small,bf]{caption}
%\setlength{\captionmargin}{20pt}
%
%\usepackage[small,compact]{titlesec}
%\usepackage[overlay,absolute]{textpos}
%\usepackage{calligra}
%\usepackage{vicent}
%\usepackage{duerer}
%\usepackage{animate}
%\usepackage{listings}
%--
%\usepackage[abs]{overpic}
%\usepackage{pict2e}
%\usepackage{mwe}
%
\usepackage{parskip}
\usepackage{enumerate}
\usepackage{url}
%\usepackage[utf8]{inputenc}
%\usepackage[super,compress]{cite}
%\usepackage{unicode}
%---
% http://en.wikibooks.org/wiki/LaTeX/Hyperlinks
\usepackage[unicode,pagebackref=true]{hyperref}
\hypersetup{ bookmarks=true, % show bookmarks bar? unicode=false, % non-Latin characters in Acrobat?s bookmarks pdftoolbar=true, % show Acrobat?s toolbar? pdfmenubar=true, % show Acrobat?s menu? pdffitwindow=false, % window fit to page when opened pdfstartview={FitH}, % fits the width of the page to the window pdftitle={My title}, % title pdfauthor={Author}, % author pdfsubject={Subject}, % subject of the document pdfcreator={Creator}, % creator of the document pdfproducer={Producer}, % producer of the document pdfkeywords={keyword1} {key2} {key3}, % list of keywords pdfnewwindow=true, % links in new PDF window colorlinks=false, % false: boxed links; true: colored links linkcolor=red, % color of internal links (change box color with linkbordercolor) citecolor=green, % color of links to bibliography filecolor=magenta, % color of file links urlcolor=cyan % color of external links }
%
%\hypersetup{
%    bookmarks=true,         % show bookmarks bar?
%    unicode=true,           % non-Latin characters in Acrobat’s bookmarks
%    pdftoolbar=true,        % show Acrobat’s toolbar?
%    pdfmenubar=true,        % show Acrobat’s menu?
%    pdffitwindow=false,     % window fit to page when opened
%    pdfstartview={FitH},    % fits the width of the page to the window
%    pdftitle={My title},    % title
%    pdfauthor={Author},     % author
%    pdfsubject={Subject},   % subject of the document
%    pdfcreator={Creator},   % creator of the document
%    pdfproducer={Producer}, % producer of the document
%    pdfkeywords={keyword1} {key2} {key3}, % list of keywords
%    pdfnewwindow=true,      % links in new PDF window
%    colorlinks=true,        % false: boxed links; true: colored links
%    linkcolor=blue,         % color of internal links (change box color with linkbordercolor)
%%    citecolor=magenta,       % color of links to bibliography
%    citecolor=OliveGreen,   % color of links to bibliography
%%    filecolor=magenta,     % color of file links
%    filecolor=Mahogany,     % color of file links
%    urlcolor=RoyalBlue      % color of external links
%%    urlcolor=cyan           % color of external links
}
\renewcommand*\backref[1]{\ifx#1\relax \else (#1) \fi}
%\biboptions{square,numbers,sort&compress}
% \usepackage[square,numbers,sort&compress]{natbib}
% \usepackage{hypernat}
%---
\hyphenation{ma-ni-pu-la-tions}
\allowdisplaybreaks
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% basic data for the eprint:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textwidth=6.5in  \textheight=8.7in
% \leftmargin=-0.8in   \topmargin=-0.20in
% \hoffset=-.85in

%% preprint number data:
%% Change the preprint number below to your institutional preprint number
\newcommand\pubdate{\today}
%% If you will submit to hep-ex, change hep-ph to hep-ex below
%% Do not change yymmnnn; this will be automatically converted
%% to the Los Alamos hep number during the submission process
\newcommand\hepnumber{hep-ph/yymmnnn}

%%  address and funding acknowledgment data:
\def\csuma{Dipartimento di Fisica Teorica, Universit\`a di Torino, Italy\\
           INFN, Sezione di Torino, Italy}
\def\csumb{Albert-Ludwigs-Universit\"at Freiburg, Physikalisches Institut\\
           D-79104, Freiburg, Germany}
\def\csumc{INFN, Sezione di Torino, Italy}
%\def\support{Work supported by MIUR under contract
%    2001023713$\_$006 and by the Research Executive Agency (REA) of the European Union
%under the Grant Agreement PITN-GA-2012-316704 (HiggsTools).}
\def\support{Work supported by the Research Executive Agency (REA) of the European Union
under the Grant Agreement PITN-GA-2012-316704 (HiggsTools).}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   document style macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Title#1{\begin{center} {\Large\bf #1 } \end{center}}
\newcommand{\Authors}[2]{\begin{center}{ \sc #1 \hspace{0.1cm} {\rm and}
\hspace{0.1cm} #2} \end{center}}
\def\Author#1{\begin{center}{ \sc #1} \end{center}}
\def\Address#1{\begin{center}{ \it #1} \end{center}}
\def\andauth{\begin{center}{and} \end{center}}
\def\submit#1{\begin{center}Submitted to {\sl #1} \end{center}}
\newcommand\pubblock{\rightline{\begin{tabular}{l} \\
         \pubdate\\  \end{tabular}}}
\newenvironment{Abstract}{\begin{quotation}  }{\end{quotation}}
\newenvironment{Presented}{\begin{quotation} \begin{center}
             Presented at the\end{center}
      \begin{center}\begin{large}}{\end{large}\end{center} \end{quotation}}
\def\Acknowledgments{\bigskip  \bigskip \begin{center}
          \large\bf Acknowledgments\end{center}}
%\def\email#1{\footnote{\color{NavyBlue}{#1}}}
%
\def\email#1{\footnote{\href{mailto:#1}{#1}}}
%
\makeatletter
\def\section{\@startsection{section}{0}{\z@}{5.5ex plus .5ex minus
 1.5ex}{2.3ex plus .2ex}{\large\bf}}
\def\subsection{\@startsection{subsection}{1}{\z@}{3.5ex plus .5ex minus
 1.5ex}{1.3ex plus .2ex}{\normalsize\bf}}
\def\subsubsection{\@startsection{subsubsection}{2}{\z@}{-3.5ex plus
-1ex minus  -.2ex}{2.3ex plus .2ex}{\normalsize\sl}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% small size table and figure captions %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\@makecaption}[2]{%
   \vskip 10pt
   \setbox\@tempboxa\hbox{\small #1: #2}
   \ifdim \wd\@tempboxa >\hsize     % IF longer than one line:
       \small #1: #2\par          %   THEN set as ordinary paragraph.
     \else                        %   ELSE  center.
       \hbox to\hsize{\hfil\box\@tempboxa\hfil}
   \fi}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macros to collapse citation numbers to ranges %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \citenum emits the plain citation number without ornament
% \citea puts it's argument into the ornamentation for citations
% thus \cite{foo} is equivalent to \citea{\citenum{foo}}
 \def\citenum#1{{\def\@cite##1##2{##1}\cite{#1}}}
\def\citea#1{\@cite{#1}{}}
%
% Collapse citation numbers to ranges.  Non-numeric and undefined labels
% are handled.  No sorting is done.  E.g., 1,3,2,3,4,5,foo,1,2,3,,4,5
% gives 1,3,2-5,foo,1-3,,4,5
\newcount\@tempcntc
\def\@citex[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \@tempcnta\z@\@tempcntb\m@ne\def\@citea{}\@cite{\@for\@citeb:=#2\do
    {\@ifundefined
       {b@\@citeb}{\@citeo\@tempcntb\m@ne\@citea\def\@citea{,}{\bf }\@warning
       {Citation `\@citeb' on page \thepage \space undefined}}%
    {\setbox\z@\hbox{\global\@tempcntc0\csname b@\@citeb\endcsname\relax}%
     \ifnum\@tempcntc=\z@ \@citeo\@tempcntb\m@ne
       \@citea\def\@citea{,}\hbox{\csname b@\@citeb\endcsname}%
     \else
      \advance\@tempcntb\@ne
      \ifnum\@tempcntb=\@tempcntc
      \else\advance\@tempcntb\m@ne\@citeo
      \@tempcnta\@tempcntc\@tempcntb\@tempcntc\fi\fi}}\@citeo}{#1}}
\def\@citeo{\ifnum\@tempcnta>\@tempcntb\else\@citea\def\@citea{,}%
  \ifnum\@tempcnta=\@tempcntb\the\@tempcnta\else
  {\advance\@tempcnta\@ne\ifnum\@tempcnta=\@tempcntb \else\def\@citea{--}\fi
    \advance\@tempcnta\m@ne\the\@tempcnta\@citea\the\@tempcntb}\fi\fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% corrects bad spacing in LaTeX multiple line equations
% replace eqnarray with Eanarray (or use abbreviations
% in econfmacros2.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newenvironment{Eqnarray}%
%   {\arraycolsep 0.14em\begin{eqnarray}}{\end{eqnarray}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  personal abbreviations and macros
%    the following package contains macros used in this document:
%--
%- Local macros
%--
\DeclareRobustCommand{\PA}{\HepParticle{A}{}{}\Xspace}
\DeclareRobustCommand{\PV}{\HepParticle{V}{}{}\Xspace}
\DeclareRobustCommand{\PX}{\HepParticle{X}{}{}\Xspace}
\DeclareRobustCommand{\PY}{\HepParticle{Y}{}{}\Xspace}
\DeclareRobustCommand{\Pf}{\HepParticle{f}{}{}\Xspace}
\DeclareRobustCommand{\PAf}{\HepAntiParticle{\Pf}{}{}\Xspace}
\DeclareRobustCommand{\PF}{\HepParticle{F}{}{}\Xspace}
\DeclareRobustCommand{\PI}{\HepParticle{I}{}{}\Xspace}
\DeclareRobustCommand{\PL}{\HepParticle{L}{}{}\Xspace}
\DeclareRobustCommand{\PG}{\HepParticle{G}{}{}\Xspace}
\DeclareRobustCommand{\PS}{\HepParticle{S}{}{}\Xspace}
\DeclareRobustCommand{\PGN}{\HepParticle{N}{}{}\Xspace}
\DeclareRobustCommand{\Phad}{\HepParticle{h}{}{}\Xspace}
\DeclareRobustCommand{\Pho}{\HepParticle{h}{1}{}\Xspace}
\DeclareRobustCommand{\Pht}{\HepParticle{h}{2}{}\Xspace}
\DeclareRobustCommand{\PQQ}{\HepParticle{Q}{}{}\Xspace}
\DeclareRobustCommand{\PQU}{\HepParticle{U}{}{}\Xspace}
\DeclareRobustCommand{\PQD}{\HepParticle{D}{}{}\Xspace}
\DeclareRobustCommand{\PP}{\HepParticle{P}{}{}\Xspace}
%
\newcommand{\PHH}{\PH\PH}
\newcommand{\PAA}{\PA\PA}
\newcommand{\PAZ}{\PA\PZ}
\newcommand{\PZA}{\PZ\PA}
\newcommand{\PZZ}{\PZ\PZ}
\newcommand{\PWW}{\PW\PW}
\newcommand{\PVV}{\PV\PV}
%
\newcommand{\EFT}{\rm{\scriptscriptstyle{EFT}}}
\newcommand{\SMEFT}{\rm{\scriptscriptstyle{SMEFT}}}
\newcommand{\THDM}{\rm{\scriptscriptstyle{THDM}}}
\newcommand{\FR}{\rm{\scriptscriptstyle{FR}}}
\newcommand{\myLO}{\mathrm{\scriptscriptstyle{LO}}}
\newcommand{\myNLO}{\mathrm{\scriptscriptstyle{NLO}}}
\newcommand{\myNNLO}{\mathrm{\scriptscriptstyle{NNLO}}}
\newcommand{\myQCD}{\mathrm{\scriptscriptstyle{QCD}}}
\newcommand{\CT}{\mathrm{CT}}
\newcommand{\dZ}{\mathrm{dZ}}
\newcommand{\OS}{\mathrm{OS}}
\newcommand{\myQED}{\mathrm{QED}}
\newcommand{\CPP}{\mathrm{CPP}}
\newcommand{\mUV}{\mathrm{UV}}
\newcommand{\mBW}{\mathrm{BW}}
\newcommand{\OFS}{\mathrm{OFS}}
\newcommand{\intf}{\mathrm{int}}
\newcommand{\mySM}{\rm{\scriptscriptstyle{SM}}}
\newcommand{\BSM}{\rm{\scriptscriptstyle{BSM}}}
\newcommand{\SESM}{\rm{\scriptscriptstyle{SESM}}}
\newcommand{\myEW}{{\scriptscriptstyle{E}\scriptscriptstyle{W}}}
\newcommand{\ssA}{{\mathrm{A}}}
\newcommand{\ssB}{{\mathrm{B}}}
\newcommand{\ssC}{{\mathrm{C}}}
\newcommand{\ssQ}{{\mathrm{Q}}}
\newcommand{\ssE}{{\mathrm{E}}}
\newcommand{\ssF}{{\mathrm{F}}}
\newcommand{\ssG}{{\mathrm{G}}}
\newcommand{\ssR}{{\mathrm{R}}}
\newcommand{\ssK}{{\mathrm{K}}}
\newcommand{\ssdR}{{\mathrm{dR}}}
\newcommand{\ssdZ}{{\mathrm{dZ}}}
\newcommand{\ssdCZ}{{\mathrm{d}{\mathcal{Z}}}}
\newcommand{\ssD}{{\mathrm{D}}}
\newcommand{\ssI}{{\mathrm{I}}}
\newcommand{\ssU}{{\mathrm{U}}}
\newcommand{\ssL}{{\mathrm{L}}}
\newcommand{\ssP}{{\mathrm{P}}}
\newcommand{\ssPR}{{\mathrm{PR}}}
\newcommand{\ssOS}{{\mathrm{OS}}}
\newcommand{\ssS}{{\mathrm{S}}}
\newcommand{\ssH}{{\mathrm{H}}}
\newcommand{\ssV}{{\mathrm{V}}}
\newcommand{\ssM}{{\mathrm{M}}}
\newcommand{\ssN}{{\mathrm{N}}}
\newcommand{\sH}{\mathrm{H}}
\newcommand{\HH}{\mathrm{HH}}
\newcommand{\VV}{\mathrm{VV}}
\newcommand{\TR}{\mathrm{TR}}
\newcommand{\ssh}{{\mathrm{h}}}
\newcommand{\mrc}{{\mathrm{c}}}
\newcommand{\mrd}{{\mathrm{d}}}
\newcommand{\mrm}{{\mathrm{m}}}
\newcommand{\mrs}{{\mathrm{s}}}
\newcommand{\mrv}{{\mathrm{v}}}
\newcommand{\mru}{{\mathrm{u}}}
\newcommand{\mrr}{{\mathrm{r}}}
\newcommand{\mrz}{{\mathrm{z}}}
\newcommand{\ssW}{{\mathrm{W}}}
\newcommand{\ssWF}{{\mathrm{WF}}}
\newcommand{\ssWW}{{\scriptscriptstyle{\PWW}}}
\newcommand{\ssZZ}{{\scriptscriptstyle{\PZZ}}}
\newcommand{\ssT}{{\mathrm{T}}}
\newcommand{\ssZ}{{\mathrm{Z}}}
\newcommand{\bqas}{\begin{eqnarray*}}
\newcommand{\eqas}{\end{eqnarray*}}
\newcommand{\nl}{\nonumber\\}
\newcommand{\nlr}{\right.\nonumber\\}
\newcommand{\cnt}[1]{{}&#1& \left.}
\def\mnew{\mpar{\hfil NEW \hfil}\ignorespaces}
\newcommand{\lpar}{\left(}                            % bracketing
\newcommand{\rpar}{\right)}
\newcommand{\lbra}{\left[\Xspace}
\newcommand{\rbra}{\Xspace\right]}
\newcommand{\lcbr}{\left\{}
\newcommand{\rcbr}{\right\}}
\newcommand{\rbrak}[1]{\lrbr#1\rrbr}
\newcommand{\bq}{\begin{equation}}                    % equationing
\newcommand{\eq}{\end{equation}}
\newcommand{\bqa}{\arraycolsep 0.14em\begin{eqnarray}}
\newcommand{\eqa}{\end{eqnarray}}
\newcommand{\ba}[1]{\begin{array}{#1}}
\newcommand{\ea}{\end{array}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bei}{\begin{itemize}}
\newcommand{\eei}{\end{itemize}}
\newcommand{\eqn}[1]{Eq.(\ref{#1})}
\newcommand{\eqns}[2]{Eqs.(\ref{#1})--(\ref{#2})}
\newcommand{\eqnss}[1]{Eqs.(\ref{#1})}
\newcommand{\eqnsc}[2]{Eqs.(\ref{#1}) and (\ref{#2})}
\newcommand{\eqnst}[3]{Eqs.(\ref{#1}), (\ref{#2}) and (\ref{#3})}
\newcommand{\eqnsf}[4]{Eqs.(\ref{#1}), (\ref{#2}), (\ref{#3}) and (\ref{#4})}
\newcommand{\eqnsv}[5]{Eqs.(\ref{#1}), (\ref{#2}), (\ref{#3}), (\ref{#4}) and (\ref{#5})}
\newcommand{\tbn}[1]{Tab.~\ref{#1}}
\newcommand{\tabn}[1]{Tab.~\ref{#1}}
\newcommand{\tbns}[2]{Tabs.~\ref{#1}--\ref{#2}}
\newcommand{\tabns}[2]{Tabs.~\ref{#1}--\ref{#2}}
\newcommand{\tabnsc}[2]{Tabs.~\ref{#1} and \ref{#2}}
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\figs}[2]{Figs.~\ref{#1}--\ref{#2}}
\newcommand{\sect}[1]{Section~\ref{#1}}
\newcommand{\sects}[2]{Section~\ref{#1} and \ref{#2}}
\newcommand{\sectm}[2]{Section~\ref{#1} -- \ref{#2}}
\newcommand{\subsect}[1]{Subsection~\ref{#1}}
\newcommand{\subsectm}[2]{Subsection~\ref{#1} -- \ref{#2}}
\newcommand{\appendx}[1]{Appendix~\ref{#1}}
\newcommand{\hsp}{\hspace{.5mm}}
\def\negs{\hspace{-0.26in}}
\def\negsh{\hspace{-0.13in}}
%--
\newcommand{\hatp}{{\hat p}}
\newcommand{\barq}{\overline q}
\newcommand{\barb}{\overline b}
\newcommand{\bmid}{\Bigr|}
\newcommand{\intrp}{\int_0^{\infty}}
\newcommand{\intMB}{\int_{-i\,\infty}^{+i\,\infty}}
\newcommand{\ord}[1]{{\cal O}\lpar#1\rpar}
\newcommand{\oD}{{\overline \Delta}}
\newcommand{\hD}{{\hat{\Delta}}}
%--
\newcommand{\Mbp}{\mathswitch {m_{\PQbpr}}}
\newcommand{\Mtp}{\mathswitch {m_{\PQtpr}}}
\newcommand{\Mlp}{\mathswitch {m_{\Pl'}}}
\newcommand{\Mnp}{\mathswitch {m_{\PGnl'}}}
\newcommand{\Bref}[1]{Ref.~\cite{#1}}
\newcommand{\Brefs}[1]{Refs.~\cite{#1}}
\newcommand{\Fref}[1]{Fig.~[#1]}
\newcommand{\Tref}[1]{Tab.~[#1]}
%--
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\etcc}{etc,\@\xspace}
\newcommand{\etal}{\emph{et al.}}
%\newcommand{\cf}{\emph{cf.\xspace}}
%\newcommand{\SPp}{~}       %% space before punctuation in math
%--
%\newcommand{\mv}{\mathswitch {M_{\ssV}}}
\newcommand{\mv}{\mathswitch{M_{\PV}}}
\newcommand{\mw}{\mathswitch{M_{\PW}}}
\newcommand{\mbw}{\mathswitch{m_{\PW}}}
\newcommand{\mbws}{\mathswitch{m^2_{\PW}}}
\newcommand{\mz}{\mathswitch{M_{\PZ}}}
\newcommand{\mBh}{\mathswitch{{\overline M}_{\PH}}}
\newcommand{\mBhs}{\mathswitch{{\overline M}^2_{\PH}}}
\newcommand{\mws}{\mathswitch{M^2_{\PW}}}
\newcommand{\mwc}{\mathswitch{M^3_{\PW}}}
\newcommand{\mwsOS}{\mathswitch{M^2_{\PW\,;\,\ssOS}}}
\newcommand{\mwq}{\mathswitch{M^4_{\PW}}}
\newcommand{\mwvi}{\mathswitch{M^6_{\PW}}}
\newcommand{\mzs}{\mathswitch{M^2_{\PZ}}}
\newcommand{\mzc}{\mathswitch{M^3_{\PZ}}}
\newcommand{\mzq}{\mathswitch{M^4_{\PZ}}}
\newcommand{\mzOS}{\mathswitch{M_{\PZ\,;\,\ssOS}}}
\newcommand{\mzsOS}{\mathswitch{M^2_{\PZ\,;\,\ssOS}}}
\newcommand{\mt}{\mathswitch{M_{\PQt}}}
\newcommand{\mb}{\mathswitch{M_{\PQb}}}
\newcommand{\mts}{\mathswitch{M^2_{\PQt}}}
\newcommand{\mbs}{\mathswitch{M^2_{\PQb}}}
\newcommand{\mtq}{\mathswitch{M^4_{\PQt}}}
\newcommand{\mbq}{\mathswitch{M^4_{\PQb}}}
\newcommand{\ml}{\mathswitch{M_{\Pl}}}
%
\newcommand{\mUs}{\mathswitch{M^2_{\PQU}}}
\newcommand{\mDs}{\mathswitch{M^2_{\PQD}}}
%
\newcommand{\smh}{\mathswitch{m_{\PH}}}
\newcommand{\mh}{\mathswitch{M_{\PH}}}
\newcommand{\mhOS}{\mathswitch{M_{\PH\,;\,\ssOS}}}
\newcommand{\mhc}{\mathswitch{M^2_{\sPH}}}
\newcommand{\mhs}{\mathswitch{M^2_{\sPH}}}
\newcommand{\mhsOS}{\mathswitch{M^2_{\PH\,;\,\ssOS}}}
\newcommand{\mhq}{\mathswitch{M^4_{\PH}}}
\newcommand{\mhvi}{\mathswitch{M^6_{\PH}}}
%
\newcommand{\mhr}{\mathswitch{M_{\PH\,\ren}}}
\newcommand{\mhrs}{\mathswitch{M^2_{\PH\,\ren}}}
%
\newcommand{\mqt}{\mathswitch{M_{\PQt}}}
\newcommand{\mqb}{\mathswitch{M_{\PQb}}}
\newcommand{\mqts}{\mathswitch{M^2_{\PQt}}}
\newcommand{\mqbs}{\mathswitch{M^2_{\PQb}}}
\newcommand{\mqtq}{\mathswitch{M^4_{\PQt}}}
\newcommand{\mqbq}{\mathswitch{M^4_{\PQb}}}
%
\newcommand{\sPF}{{\scriptscriptstyle{\PF}}}
\newcommand{\sPQQ}{{\scriptscriptstyle{\PQQ}}}
\newcommand{\sPL}{{\scriptscriptstyle{\PL}}}
\newcommand{\sPQU}{{\scriptscriptstyle{\PQU}}}
\newcommand{\sPQD}{{\scriptscriptstyle{\PQD}}}
\newcommand{\sPH}{{\scriptscriptstyle{\PH}}}
\newcommand{\sPS}{{\scriptscriptstyle{\PS}}}
\newcommand{\sPZ}{{\scriptscriptstyle{\PZ}}}
\newcommand{\sPW}{{\scriptscriptstyle{\PW}}}
\newcommand{\sPA}{{\scriptscriptstyle{\PA}}}
\newcommand{\sPB}{{\scriptscriptstyle{\PB}}}
\newcommand{\sPD}{{\scriptscriptstyle{\PD}}}
\newcommand{\sPP}{{\scriptscriptstyle{\PP}}}
\newcommand{\sPV}{{\scriptscriptstyle{\PV}}}
\newcommand{\sPVV}{{\scriptscriptstyle{\PV\PV}}}
\newcommand{\sPZZ}{{\scriptscriptstyle{\PZZ}}}
\newcommand{\sPWW}{{\scriptscriptstyle{\PWW}}}
\newcommand{\sPHAA}{{\scriptscriptstyle{\PH\PAA}}}
\newcommand{\sPHAZ}{{\scriptscriptstyle{\PH\PA\PZ}}}
\newcommand{\sPHAV}{{\scriptscriptstyle{\PH\PA\PV}}}
\newcommand{\sPHZZ}{{\scriptscriptstyle{\PH\PZ\PZ}}}
\newcommand{\sPHWW}{{\scriptscriptstyle{\PH\PW\PW}}}
\newcommand{\sPHVV}{{\scriptscriptstyle{\PH\PV\PV}}}
%
\newcommand{\smu}{\mathswitch{m_{\PQu}}}
\newcommand{\smU}{\mathswitch{m_{\sPQU}}}
\newcommand{\mqu}{\mathswitch{M_{\PQu}}}
\newcommand{\mqU}{\mathswitch{M_{\sPQU}}}
\newcommand{\mqus}{\mathswitch{M^2_{\PQu}}}
\newcommand{\mquq}{\mathswitch{M^4_{\PQu}}}
\newcommand{\mqd}{\mathswitch{M_{\PQd}}}
\newcommand{\mqD}{\mathswitch{M_{\sPQD}}}
\newcommand{\smd}{\mathswitch{m_{\PQd}}}
\newcommand{\smD}{\mathswitch{m_{\sPQD}}}
\newcommand{\mqds}{\mathswitch{M^2_{\PQd}}}
\newcommand{\mqdq}{\mathswitch{M^4_{\PQd}}}
\newcommand{\smLe}{\mathswitch{m_{\sPL}}}
\newcommand{\smle}{\mathswitch{m_{\Pl}}}
\newcommand{\mle}{\mathswitch{M_{\Pl}}}
\newcommand{\mLe}{\mathswitch{M_{\sPL}}}
\newcommand{\mLes}{\mathswitch{M^2_{\sPL}}}
\newcommand{\mles}{\mathswitch{M^2_{\Pl}}}
\newcommand{\mleq}{\mathswitch{M^4_{\Pl}}}
%
\newcommand{\cph}{\mathswitch{s_{\sPH}}}
\newcommand{\cpw}{\mathswitch{s_{\sPW}}}
\newcommand{\cpwz}{\mathswitch{s_{\PW}, s_{\PZ}}}
\newcommand{\cpz}{\mathswitch{s_{\sPZ}}}
\newcommand{\cpt}{\mathswitch{s_{\PQt}}}
\newcommand{\muh}{\mathswitch{\mu_{\PH}}}
\newcommand{\muph}{\mathswitch{\mu'_{\PH}}}
\newcommand{\muhs}{\mathswitch{\mu^2_{\PH}}}
\newcommand{\omuhs}{\mathswitch{{\hat\mu}^2_{\PH}}}
\newcommand{\gh}{\mathswitch{\gamma_{\PH}}}
\newcommand{\emc}{\mathswitch{\gamma}}
\newcommand{\emcb}{\mathswitch{{\overline{\gamma}}}}
\newcommand{\GOS}{\mathswitch{\Gamma_{\OS}}}
\newcommand{\GOL}{\mathswitch{\overline\Gamma}}
\newcommand{\muol}{\mathswitch{\overline\mu}}
\newcommand{\GOSu}{\mathswitch{\Gamma^{\OS}}}
\newcommand{\shat}{\mathswitch{\hat s}}
\newcommand{\muR}{\mathswitch{\mu_{\ssR}}}
\newcommand{\muF}{\mathswitch{\mu_{\ssF}}}
\newcommand{\muRs}{\mathswitch{\mu^2_{\ssR}}}
\newcommand{\muFs}{\mathswitch{\mu^2_{\ssF}}}
\newcommand{\tot}{{\mbox{\scriptsize tot}}}
\newcommand{\myprod}{{\mbox{\scriptsize prod}}}
%%%%\newcommand{\prop}{{\mbox{\scriptsize prop}}}
\newcommand{\proc}{{\mbox{\scriptsize proc}}}
\newcommand{\dec}{{\mbox{\scriptsize dec}}}
\newcommand{\off}{{\mbox{\scriptsize off}}}
\newcommand{\obs}{{\mbox{\scriptsize obs}}}
\newcommand{\kcut}{{\mbox{\scriptsize cut}}}
\newcommand{\bck}{{\mbox{\scriptsize NR}}}
\newcommand{\res}{{\mbox{\scriptsize R}}}
\newcommand{\mysoft}{{\mbox{\scriptsize soft}}}
\newcommand{\ch}{{\mbox{\scriptsize ch}}}
\newcommand{\inv}{{\mbox{\scriptsize inv}}}
\newcommand{\bos}{{\mbox{\scriptsize bos}}}
\newcommand{\peak}{{\mbox{\scriptsize peak}}}
\newcommand{\eff}{{\mbox{\scriptsize eff}}}
\newcommand{\rest}{{\mbox{\scriptsize rest}}}
\newcommand{\bare}{{\mbox{\scriptsize bare}}}
\newcommand{\tree}{{\mbox{\scriptsize tree}}}
\newcommand{\icdiv}{{\mbox{\scriptsize div}}}
\newcommand{\oL}{{\mbox{\scriptsize 1L}}}
\newcommand{\real}{{\mbox{\scriptsize real}}}
\newcommand{\myvirt}{{\mbox{\scriptsize virt}}}
%\newcommand{\fin}{{\mbox{\scriptsize fin}}}
\newcommand{\fin}{{\mbox{\tiny fin}}}
\newcommand{\pole}{{\mbox{\tiny div}}}
\newcommand{\gen}{{\mbox{\scriptsize gen}}}
\newcommand{\ggen}{{\mbox{\tiny gen}}}
\newcommand{\ren}{{\mbox{\scriptsize ren}}}
\newcommand{\ct}{{\mbox{\scriptsize ct}}}
\newcommand{\mdiv}{{\mbox{\scriptsize div}}}
\newcommand{\bin}{{\mbox{\scriptsize in}}}
\newcommand{\bout}{{\mbox{\scriptsize out}}}
\newcommand{\ac}{{\mbox{\scriptsize all}}}
\newcommand{\HO}{{\mathrm{HO}}}
\newcommand{\intfxy}[2]{\int_{\scriptstyle 0}^{\scriptstyle 1}\,d#1\,
                        \int_{\scriptstyle 0}^{\scriptstyle #1}\,d#2}
\newcommand{\li}[2]{\mathrm{Li}_{#1}\lpar\displaystyle{#2}\rpar} % polylog
%--
\newcommand{\eG}[1]{\mathswitch \Gamma\lpar #1 \rpar}
\newcommand{\eGs}[1]{\mathswitch \Gamma^2\lpar #1 \rpar}
\newcommand{\ep}{\mathswitch \varepsilon}
\newcommand{\epb}{\mathswitch{\overline\varepsilon}}
\newcommand{\eph}{\mathswitch{\hat\varepsilon}}
\newcommand{\spro}[2]{{#1}\cdot{#2}}
\providecommand\HTO{{\sc HTO}}
\providecommand\POWHEG{{\sc POWHEG}}
\providecommand\iHixs{{\sc iHixs}}
%--
\newcommand{\Srest}[2]{\sigma_{#1}\lpar{#2}\rpar}
\newcommand{\Gdist}[1]{{\mathcal{G}}\lpar{#1}\rpar}
\newcommand{\resolw}{\sigma_{\ssE}}
\newcommand{\resolws}{\sigma^2_{\ssE}}
\newcommand{\ddel}[1]{\delta\lpar#1\rpar}
\newcommand{\Gloni}[1]{\Gamma_{#1}}
\newcommand{\Aareai}[1]{{\mathcal{A}}\lpar{#1}\rpar}
\newcommand{\lrbr}{\left[}
\newcommand{\rrbr}{\right]}
%\newcommand{\lcbr}{\left\{}
%\newcommand{\rcbr}{\right\}}
\newcommand{\sGdist}{{\mathcal{G}}}
\newcommand{\sAarea}{{\mathcal{A}}}
%--
\newcommand{\Ds}{{\mathrm{D}}}
\newcommand{\mrS}{{\mathrm{S}}}
\newcommand{\mrA}{{\mathrm{A}}}
%\newcommand{\mrA}{{{\overline{\mathrm{A}}}}}
\newcommand{\mrB}{{\mathrm{B}}}
\newcommand{\mrC}{{\mathrm{C}}}
\newcommand{\mrD}{{\mathrm{D}}}
\newcommand{\mrE}{{\mathrm{E}}}
\newcommand{\mrF}{{\mathrm{F}}}
\newcommand{\mrG}{{\mathrm{G}}}
\newcommand{\mrH}{{\mathrm{H}}}
\newcommand{\mrI}{{\mathrm{I}}}
\newcommand{\mrJ}{{\mathrm{J}}}
\newcommand{\mrK}{{\mathrm{K}}}
\newcommand{\mrL}{{\mathrm{L}}}
\newcommand{\mrM}{{\mathrm{M}}}
\newcommand{\mrN}{{\mathrm{N}}}
\newcommand{\mrO}{{\mathrm{O}}}
\newcommand{\mrP}{{\mathrm{P}}}
\newcommand{\mrQ}{{\mathrm{Q}}}
\newcommand{\mrR}{{\mathrm{R}}}
%\newcommand{\mrS}{{\mathrm{S}}}
\newcommand{\mrT}{{\mathrm{T}}}
\newcommand{\mrU}{{\mathrm{U}}}
\newcommand{\mrV}{{\mathrm{V}}}
\newcommand{\mrW}{{\mathrm{W}}}
\newcommand{\mrw}{{\mathrm{w}}}
\newcommand{\mrX}{{\mathrm{X}}}
\newcommand{\mrZ}{{\mathrm{Z}}}
%\newcommand{\mrW}{{\mathrm{W}}}
%--
\newcommand{\Lcol}{{\mrL_c}}
\newcommand{\LM}{{\mrL}}
%
\newcommand{\Kfac}[2]{\mathrm{K}^{#1}_{#2}}
\newcommand{\Kf}{\mathrm{K}}
\newcommand{\SpI}{\mathrm{S} + \mathrm{I}}
\newcommand{\mfs}{\mathswitch{M_{\Pf}}}
%--
\newcommand{\cmark}{\ding{51}\Xspace}
\newcommand{\ccmark}{\ding{55}\Xspace}
\newcommand{\quo}{\ding{125}\Xspace}
\newcommand{\uquo}{\ding{126}\Xspace}
\newcommand{\bhand}{{\Large{\ding{42}}}\Xspace}
\newcommand{\whand}{{\Large{\ding{43}}}\Xspace}
\newcommand{\vict}{{\Large{\ding{44}}}\Xspace}
\newcommand{\far}{{\Large{\ding{243}}}\Xspace}
\newcommand{\dstar}{{\Large{\ding{85}}}\Xspace}
\newcommand{\apdown}{{\Large{\ding{244}}}\Xspace}
\newcommand{\sciss}{{\Large{\ding{34}}}\Xspace}
\newcommand{\dcross}{{\Huge{\ding{54}}}\Xspace}
\newcommand{\pwrite}{{\Huge{\ding{46}}}\Xspace}
%
\providecommand{\dnuma}{{\Large{\ding{172}}}\Xspace}
\providecommand{\dnumb}{{\Large{\ding{173}}}\Xspace}
\providecommand{\dnumc}{{\Large{\ding{174}}}\Xspace}
\providecommand{\dnumd}{{\Large{\ding{175}}}\Xspace}
%--
%%%%\newtheorem{theorem}{Theorem}[section]
%%%%\newtheorem{lemma}[theorem]{Lemma}
%%%%\newtheorem{proposition}[theorem]{Proposition}
%%%%\newtheorem{corollary}[theorem]{Corollary}

%%%%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%%%%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%%%%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%%%%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%%%%\newenvironment{example}[1][Example]{\begin{trivlist}
%%%%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%%%%\newenvironment{remark}[1][Remark]{\begin{trivlist}
%%%%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%
%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{definition}[1][Definition]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{claim}[1][Claim]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%
\newcommand{\Lag}{{\cal L}}
\newcommand{\Ope}{{\cal O}}
\newcommand{\Amp}{{\cal M}}
\newcommand{\srt}{\sqrt{2}}
%
\newcommand{\OpWs}{\Ope^{(6)}_{\upphi\,\scriptscriptstyle{\PW}}}
\newcommand{\OpWe}{\Ope^{(8)}_{\upphi\,\scriptscriptstyle{\PW}}}
%
\DeclareRobustCommand{\POppm}{\HepAntiParticle{\upphi}{}{\,\pm}\Xspace}
\DeclareRobustCommand{\POpp}{\HepAntiParticle{\upphi}{}{\,+}\Xspace}
\DeclareRobustCommand{\POpm}{\HepAntiParticle{\upphi}{}{\,-}\Xspace}
\DeclareRobustCommand{\POpz}{\HepAntiParticle{\upphi}{}{\,0}\Xspace}
%--
\DeclareRobustCommand{\Ppp}{\HepParticle{\upphi}{}{+}\Xspace}
\DeclareRobustCommand{\Ppm}{\HepParticle{\upphi}{}{-}\Xspace}
\DeclareRobustCommand{\Pppm}{\HepParticle{\upphi}{}{\pm}\Xspace}
\DeclareRobustCommand{\Ppz}{\HepParticle{\upphi}{}{0}\Xspace}
%
\DeclareRobustCommand{\PAL}{\HepParticle{\mybar{\PL}}{}{}\Xspace}
\DeclareRobustCommand{\PpsiL}{\HepParticle{\uppsi}{L}{}\Xspace}
\DeclareRobustCommand{\PpsiR}{\HepParticle{\uppsi}{R}{}\Xspace}
\DeclareRobustCommand{\POpsiL}{\HepParticle{\mybar{\uppsi}}{L}{}\Xspace}
\DeclareRobustCommand{\POpsiR}{\HepParticle{\mybar{\uppsi}}{R}{}\Xspace}
\DeclareRobustCommand{\PQtR}{\HepParticle{\PQt}{R}{}\Xspace}
\DeclareRobustCommand{\PQbR}{\HepParticle{\PQb}{R}{}\Xspace}
\DeclareRobustCommand{\PQuR}{\HepParticle{\PQu}{R}{}\Xspace}
\DeclareRobustCommand{\PQdR}{\HepParticle{\PQd}{R}{}\Xspace}
\DeclareRobustCommand{\PQqL}{\HepParticle{\PQq}{L}{}\Xspace}
\DeclareRobustCommand{\PlL}{\HepParticle{\Pl}{L}{}\Xspace}
\DeclareRobustCommand{\PlR}{\HepParticle{\Pl}{R}{}\Xspace}
\DeclareRobustCommand{\PLL}{\HepParticle{\PL}{L}{}\Xspace}
\DeclareRobustCommand{\PLR}{\HepParticle{\PL}{R}{}\Xspace}
\DeclareRobustCommand{\PAQqL}{\HepParticle{\PAQq}{L}{}\Xspace}
\DeclareRobustCommand{\PAlL}{\HepParticle{\PAl}{L}{}\Xspace}
\DeclareRobustCommand{\PAlR}{\HepParticle{\PAl}{R}{}\Xspace}
\DeclareRobustCommand{\PALL}{\HepParticle{\PAL}{L}{}\Xspace}
\DeclareRobustCommand{\PAQuR}{\HepParticle{\PAQu}{R}{}\Xspace}
\DeclareRobustCommand{\PAQdR}{\HepParticle{\PAQd}{R}{}\Xspace}
%-
\newcommand{\pumu}{{\partial^{\mu}}}
%\newcommand{\pdmu}{{\partial_{\mu}}}
%\newcommand{\punu}{{\partial^{\nu}}}
\newcommand{\pdnu}{{\partial_{\nu}}}
%
\newcommand{\myGF}{G_{\mrF}}
%
%\DeclareRobustCommand{\PK}{\HepParticle{K}{}{}\Xspace}
%\DeclareRobustCommand{\Pphi}{\HepParticle{\upphi}{}{}\Xspace}
%\DeclareRobustCommand{\PKdag}{\HepParticle{\PK}{}{\dagger}\Xspace}
%\newcommand{\KdK}{\lpar \PKdag\,\PK\rpar }
%
\DeclareRobustCommand{\PK}{\HepParticle{\upPhi}{}{}\Xspace}
\DeclareRobustCommand{\Pphi}{\HepParticle{\upphi}{}{}\Xspace}
\DeclareRobustCommand{\PKdag}{\HepParticle{\PK}{}{\dagger}\Xspace}
\newcommand{\KdK}{\lpar \PKdag\,\PK\rpar }
%
\DeclareRobustCommand{\Pxi}{\HepParticle{\upxi}{}{}\Xspace}
\DeclareRobustCommand{\Pxip}{\HepParticle{\upxi}{}{+}\Xspace}
\DeclareRobustCommand{\Pxim}{\HepParticle{\upxi}{}{-}\Xspace}
\DeclareRobustCommand{\Pxiz}{\HepParticle{\upxi}{}{0}\Xspace}
\DeclareRobustCommand{\Pxid}{\HepParticle{\upxi}{}{\dagger}\Xspace}
%
\newcommand{\dPK}{{\partial\PK}}
\newcommand{\essV}{{\mathrm{e}\PV}}
\DeclareRobustCommand{\PAf}{\HepAntiParticle{\Pf}{}{}\Xspace}
%
%\newcommand{\mrc}{\mathrm{c}}
%\newcommand{\mrs}{\mathrm{s}}
%
\newcommand{\stse}{\sin\theta^{\Pf}_{\eff}}
%
\newcommand{\sa}{\mrs_{_{\alpha}}}
\newcommand{\ca}{\mrc_{_{\alpha}}}
%
\newcommand{\stw}{\mrs_{_{\theta}}}             % bare, Lagrangian parameters
\newcommand{\ctw}{\mrc_{_{\theta}}}
\newcommand{\stws}{\mrs_{_{\theta}}^2}
\newcommand{\ctws}{\mrc_{_{\theta}}^2}
\newcommand{\ctwc}{\mrc_{_{\theta}}^3}
\newcommand{\stwq}{\mrs_{_{\theta}}^4}
\newcommand{\ctwq}{\mrc_{_{\theta}}^4}
\newcommand{\stwvi}{\mrs_{_{\theta}}^6}
\newcommand{\ctwvi}{\mrc_{_{\theta}}^6}
%
\newcommand{\ctwr}{\mrc^{\ren}_{_{\theta}}}
\newcommand{\stwr}{s^{\ren}_{_{\theta}}}
%
\newcommand{\stW}{\mrs_{_{\PW}}}             % bare, Lagrangian parameters
\newcommand{\ctW}{\mrc_{_{\PW}}}
\newcommand{\stWs}{\mrs_{_{\PW}}^2}
\newcommand{\ctWs}{\mrc_{_{\PW}}^2}
\newcommand{\ctWc}{\mrc_{_{\PW}}^3}
\newcommand{\stWq}{\mrs_{_{\PW}}^4}
\newcommand{\ctWq}{\mrc_{_{\PW}}^4}
\newcommand{\stWvi}{\mrs_{_{\PW}}^6}
\newcommand{\ctWvi}{\mrc_{_{\PW}}^6}
%--
\newcommand{\ctb}{\overline{\mrc}_{_{\theta}}}
\newcommand{\stb}{\overline{\mrs}_{_{\theta}}}
\newcommand{\ctbs}{\overline{\mrc}^2_{_{\theta}}}
\newcommand{\stbs}{\overline{\mrs}^2_{_{\theta}}}
%
\newcommand\mybar[1]{\ensuremath{\bar{#1}}}
\newcommand\mytil[1]{\ensuremath{\tilde{#1}}}
%
\newcommand{\cth}{{\hat \mrc}_{_{\theta}}}
\newcommand{\sth}{{\hat \mrs}_{_{\theta}}}
\newcommand{\cths}{{\hat \mrc}^2_{_{\theta}}}
\newcommand{\cthc}{{\hat \mrc}^3_{_{\theta}}}
\newcommand{\sths}{{\hat \mrs}^2_{_{\theta}}}
\newcommand{\sthq}{{\hat \mrs}^4_{_{\theta}}}
%
\newcommand{\HSs}{{\Lambda^2}}
%
\DeclareRobustCommand{\PWp}{\HepParticle{\PW}{}{+}\Xspace}
\DeclareRobustCommand{\PWm}{\HepParticle{\PW}{}{-}\Xspace}
\DeclareRobustCommand{\PWpmmu}{\HepParticle{\PW}{\mu}{\pm}\Xspace}
\DeclareRobustCommand{\PWpmu}{\HepParticle{\PW}{\mu}{+}\Xspace}
\DeclareRobustCommand{\PWmmu}{\HepParticle{\PW}{\mu}{-}\Xspace}
\DeclareRobustCommand{\PWpnu}{\HepParticle{\PW}{\nu}{+}\Xspace}
\DeclareRobustCommand{\PWmnu}{\HepParticle{\PW}{\nu}{-}\Xspace}
\DeclareRobustCommand{\PZmu}{\HepParticle{\PZ}{\mu}{}\Xspace}
\DeclareRobustCommand{\PAmu}{\HepParticle{\PA}{\mu}{}\Xspace}
\DeclareRobustCommand{\PZnu}{\HepParticle{\PZ}{\nu}{}\Xspace}
\DeclareRobustCommand{\PAnu}{\HepParticle{\PA}{\nu}{}\Xspace}
%
\DeclareRobustCommand{\PAumu}{\HepParticle{\PA}{}{\mu}\Xspace}
\DeclareRobustCommand{\PAdmu}{\HepParticle{\PA}{\mu}{}\Xspace}
%
\DeclareRobustCommand{\PZumu}{\HepParticle{\PZ}{}{\mu}\Xspace}
\DeclareRobustCommand{\PZdmu}{\HepParticle{\PZ}{\mu}{}\Xspace}
%\DeclareRobustCommand{\PZdmus}{\HepParticle{\PZ}{\mu}{}\Xspace}
\DeclareRobustCommand{\PZunu}{\HepParticle{\PZ}{}{\nu}\Xspace}
\DeclareRobustCommand{\PZdnu}{\HepParticle{\PZ}{\nu}{}\Xspace}
%
\DeclareRobustCommand{\PAumu}{\HepParticle{\PA}{}{\mu}\Xspace}
\DeclareRobustCommand{\PAdmu}{\HepParticle{\PA}{\mu}{}\Xspace}
\DeclareRobustCommand{\PAunu}{\HepParticle{\PA}{}{\nu}\Xspace}
\DeclareRobustCommand{\PAdnu}{\HepParticle{\PA}{\nu}{}\Xspace}
%
\DeclareRobustCommand{\PWpumu}{\HepParticle{\PW}{}{+\,\mu}\Xspace}
\DeclareRobustCommand{\PWmdmu}{\HepParticle{\PW}{\mu}{-}\Xspace}
\DeclareRobustCommand{\PWpunu}{\HepParticle{\PW}{}{+\,\nu}\Xspace}
\DeclareRobustCommand{\PWmdnu}{\HepParticle{\PW}{\nu}{-}\Xspace}
%
\DeclareRobustCommand{\PWmumu}{\HepParticle{\PW}{}{-\,\mu}\Xspace}
\DeclareRobustCommand{\PWpdmu}{\HepParticle{\PW}{\mu}{+}\Xspace}
\DeclareRobustCommand{\PWmunu}{\HepParticle{\PW}{}{-\,\nu}\Xspace}
\DeclareRobustCommand{\PWpdnu}{\HepParticle{\PW}{\nu}{+}\Xspace}
%--
\DeclareRobustCommand{\PXpm}{\HepParticle{\PX}{}{\pm}\Xspace}
\DeclareRobustCommand{\PXp}{\HepParticle{\PX}{}{+}\Xspace}
\DeclareRobustCommand{\PXm}{\HepParticle{\PX}{}{-}\Xspace}
\DeclareRobustCommand{\PYz}{\HepParticle{\PY}{\PZ}{}\Xspace}
\DeclareRobustCommand{\PYa}{\HepParticle{\PY}{\PA}{}\Xspace}
%
\DeclareRobustCommand{\PHb}{\HepAntiParticle{\PH}{}{}\Xspace}
\DeclareRobustCommand{\Ppzb}{\HepAntiParticle{\upphi}{}{\,0}\Xspace}
\DeclareRobustCommand{\Pppmb}{\HepAntiParticle{\upphi}{}{\pm}\Xspace}
\DeclareRobustCommand{\PAb}{\HepAntiParticle{\PA}{}{}\Xspace}
\DeclareRobustCommand{\PAbmu}{\HepAntiParticle{\PA}{}{\mu}\Xspace}
\DeclareRobustCommand{\PAbmud}{\HepAntiParticle{\PA}{\mu}{}\Xspace}
\DeclareRobustCommand{\PZb}{\HepAntiParticle{\PZ}{}{}\Xspace}
\DeclareRobustCommand{\PZbmu}{\HepAntiParticle{\PZ}{}{\mu}\Xspace}
\DeclareRobustCommand{\PZbmud}{\HepAntiParticle{\PZ}{\mu}{}\Xspace}
%
\DeclareRobustCommand{\PWpmbmu}{\HepAntiParticle{\PW}{}{\pm\,\mu}\Xspace}
\DeclareRobustCommand{\PWpmbmud}{\HepAntiParticle{\PW}{\mu}{\pm}\Xspace}
\DeclareRobustCommand{\PWb}{\HepAntiParticle{\PW}{}{}\Xspace}
\DeclareRobustCommand{\PWpb}{\HepAntiParticle{\PW}{}{+}\Xspace}
\DeclareRobustCommand{\PWmb}{\HepAntiParticle{\PW}{}{-}\Xspace}
\DeclareRobustCommand{\Pgb}{\HepAntiParticle{\Pg}{}{}\Xspace}
\DeclareRobustCommand{\PQtb}{\HepAntiParticle{\PQt}{}{}\Xspace}
\DeclareRobustCommand{\PQbb}{\HepAntiParticle{\PQb}{}{}\Xspace}
\DeclareRobustCommand{\PXpmb}{\HepAntiParticle{\PX}{}{\pm}\Xspace}
\DeclareRobustCommand{\PYzb}{\HepAntiParticle{\PY}{\PZ}{}\Xspace}
\DeclareRobustCommand{\PYab}{\HepAntiParticle{\PY}{\PA}{}\Xspace}
%
\DeclareRobustCommand{\PAXpm}{\HepAntiParticle{\PX}{}{\,\pm}\Xspace}
\DeclareRobustCommand{\PAXp}{\HepAntiParticle{\PX}{}{\,+}\Xspace}
\DeclareRobustCommand{\PAXm}{\HepAntiParticle{\PX}{}{\,-}\Xspace}
\DeclareRobustCommand{\PAYz}{\HepAntiParticle{\PY}{\,\PZ}{}\Xspace}
\DeclareRobustCommand{\PAYa}{\HepAntiParticle{\PY}{\,\PA}{}\Xspace}
%
\newcommand{\POZ}{{\overline{\PZ}}}
\newcommand{\POA}{{\overline{\PA}}}
\newcommand{\POH}{{\overline{\PH}}}
\newcommand{\POp}{{\overline{\upphi}}}
%--
\DeclareRobustCommand{\PdT}{\HepParticle{\mytil{\PF}}{\mu\nu}{a}\Xspace}
\DeclareRobustCommand{\HB}{\HepAntiParticle{\PH}{}{}\Xspace}
\DeclareRobustCommand{\PZB}{\HepAntiParticle{\PZ}{}{}\Xspace}
\DeclareRobustCommand{\myPAB}{\HepAntiParticle{\PA}{}{}\Xspace}
\DeclareRobustCommand{\OM}{\HepAntiParticle{\PM}{}{}\Xspace}
\DeclareRobustCommand{\OMf}{\HepAntiParticle{\PM}{}{\Pf}\Xspace}
\DeclareRobustCommand{\OMs}{\HepAntiParticle{\PM}{}{\,2}\Xspace}
\DeclareRobustCommand{\OMq}{\HepAntiParticle{\PM}{}{\,4}\Xspace}
\DeclareRobustCommand{\OMzs}{\HepAntiParticle{\PM}{\,0}{\,2}\Xspace}
\DeclareRobustCommand{\OMzq}{\HepAntiParticle{\PM}{\,0}{\,4}\Xspace}
\DeclareRobustCommand{\OMH}{\HepAntiParticle{\PM}{\,\PH}{}\Xspace}
\DeclareRobustCommand{\OMHs}{\HepAntiParticle{\PM}{\,\PH}{\,2}\Xspace}
\DeclareRobustCommand{\OMHq}{\HepAntiParticle{\PM}{\,\PH}{\,4}\Xspace}
\DeclareRobustCommand{\phib}{\HepAntiParticle{\upphi}{}{}\Xspace}
\newcommand{\ACf}{\frac{\OMs}{\HSs}}
%
%
\newcommand{\myYM}{\rm{\scriptscriptstyle{YM}}}
\newcommand{\gfix}{{\mbox{\scriptsize gf}}}
\newcommand{\myFP}{\rm{\scriptscriptstyle{FP}}}
%
\newcommand{\fact}{{\mbox{\scriptsize fc}}}
\newcommand{\nfact}{{\mbox{\scriptsize nfc}}}
\newcommand{\spin}{{\mbox{\scriptsize spin}}}
\newcommand{\app}{{\mbox{\scriptsize app}}}
\newcommand{\fer}{{\mbox{\scriptsize fer}}}
%
\DeclareRobustCommand{\OMzs}{\HepAntiParticle{\PM}{\,0}{\,2}\Xspace}
\DeclareRobustCommand{\PM}{\HepParticle{M}{}{}\Xspace}
%
\newcommand{\rmD}{\mathrm{D}}
\newcommand{\bh}{\beta_{\mathrm{h}}}
\newcommand{\bhb}{\overline{\beta}_{\mathrm{h}}}
\newcommand{\RL}{\mathrm{R}_{\Lambda}}
\newcommand{\Ddmu}{\ssD^{(\leftrightarrow)}_{\mu}}
\newcommand{\ddmu}{{\stackrel{\leftrightarrow}{\partial}}_{\mu}}
\newcommand{\drmu}{{\stackrel{\rightarrow}{\partial}}_{\mu}}
\newcommand{\dlmu}{{\stackrel{\leftarrow}{\partial}}_{\mu}}
%
\newcommand{\Mbs}{M^2}
\newcommand{\Mbc}{M^3}
\newcommand{\Mbq}{M^4}
\newcommand{\mzb}{M_0}
\newcommand{\Mzbs}{M^2_0}
\newcommand{\Mzbq}{M^q_0}
%
\newcommand{\apLWt}{a^{(3)}_{\upphi\,\sPL\,\scriptscriptstyle{\PW}}}
%
\newcommand{\apLldQ}{a_{\upphi\,\PL\Pl\PQd\PQQ}}
\newcommand{\apN}{a_{\upphi\,\PN}}
\newcommand{\aplVA}{a_{\upphi\,\Pl\,\scriptscriptstyle{\PV\PA}}}
\newcommand{\apLVA}{a_{\upphi\,\sPL\,\scriptscriptstyle{\PV\PA}}}
\newcommand{\apLA}{a_{\upphi\,\sPL\,\scriptscriptstyle{\PA}}}
\newcommand{\apLV}{a_{\upphi\,\sPL\,\scriptscriptstyle{\PV}}}
\newcommand{\apuVA}{a_{\upphi\,\PQu\,\scriptscriptstyle{\PV\PA}}}
\newcommand{\apdVA}{a_{\upphi\,\PQd\,\scriptscriptstyle{\PV\PA}}}
\newcommand{\apUVA}{a_{\upphi\,\sPQU\,\scriptscriptstyle{\PV\PA}}}
\newcommand{\apDVA}{a_{\upphi\,\sPQD\,\scriptscriptstyle{\PV\PA}}}
%
\newcommand{\apWAB}{a_{\upphi\,\scriptscriptstyle{\PW\PA\PB}}}
\newcommand{\apWAD}{a_{\upphi\,\scriptscriptstyle{\PW\PA\PD}}}
%
\newcommand{\alpBox}{a_{\Pl\,\upphi\,\scriptscriptstyle{\Box}}}
\newcommand{\aLpBox}{a_{\sPL\,\upphi\,\scriptscriptstyle{\Box}}}
\newcommand{\aupBox}{a_{\PQu\,\upphi\,\scriptscriptstyle{\Box}}}
\newcommand{\adpBox}{a_{\PQd\,\upphi\,\scriptscriptstyle{\Box}}}
%
\newcommand{\aQW}{a_{\scriptscriptstyle{\PQQ\PW}}}
\newcommand{\aAA}{a_{\scriptscriptstyle{\PAA}}}
\newcommand{\aZZ}{a_{\scriptscriptstyle{\PZZ}}}
\newcommand{\aAZ}{a_{\scriptscriptstyle{\PAZ}}}
\newcommand{\ap}{a_{\upphi}}
\newcommand{\apBox}{a_{\upphi\,\scriptscriptstyle{\Box}}}
\newcommand{\apWB}{a_{\upphi\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\apWBa}{a^{(a)}_{\upphi\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\apWDpB}{a^{(+)}_{\upphi\,\scriptscriptstyle{\PW\PD\PB}}}
\newcommand{\apWDmB}{a^{(-)}_{\upphi\,\scriptscriptstyle{\PW\PD\PB}}}
\newcommand{\apBW}{a_{\upphi\,\scriptscriptstyle{\PB\PW}}}
\newcommand{\apWA}{a_{\upphi\,\scriptscriptstyle{\PW\PA}}}
\newcommand{\apWZ}{a_{\upphi\,\scriptscriptstyle{\PW\PZ}}}
\newcommand{\apB}{a_{\upphi\,\scriptscriptstyle{\PB}}}
\newcommand{\apW}{a_{\upphi\,\scriptscriptstyle{\PW}}}
\newcommand{\apD}{a_{\upphi\,\scriptscriptstyle{\PD}}}
\newcommand{\apDB}{a_{\upphi\,\scriptscriptstyle{\PD\PB}}}
\newcommand{\apG}{a_{\upphi\,\scriptscriptstyle{\PG}}}
\newcommand{\aspG}{a^2_{\upphi\,\scriptscriptstyle{\PG}}}
%
\newcommand{\aqp}{a_{\PQq\,\upphi}}
\newcommand{\alp}{a_{\Pl\,\upphi}}
\newcommand{\aup}{a_{\PQu\,\upphi}}
\newcommand{\atp}{a_{\PQt\,\upphi}}
\newcommand{\adp}{a_{\PQd\,\upphi}}
\newcommand{\abp}{a_{\PQb\,\upphi}}
%--
\newcommand{\atG}{a_{\PQt\,\Pg}}
\newcommand{\abG}{a_{\PQb\,\Pg}}
%--
\newcommand{\aNa}{a^{(1)}_{\ssN}}
\newcommand{\aNb}{a^{(2)}_{\ssN}}
\newcommand{\aNc}{a^{(3)}_{\ssN}}
%
\newcommand{\aLp}{a_{\sPL\,\upphi}}
\newcommand{\aUp}{a_{\sPQU\,\upphi}}
\newcommand{\aDp}{a_{\sPQD\,\upphi}}
%
\newcommand{\apWDm}{a^{(-)}_{\upphi\,\scriptscriptstyle{\PW\PD}}}
\newcommand{\apWDp}{a^{(+)}_{\upphi\,\scriptscriptstyle{\PW\PD}}}
%
\newcommand{\auG}{a_{\PQu\,\scriptscriptstyle{\PG}}}
\newcommand{\adG}{a_{\PQd\,\scriptscriptstyle{\PG}}}
%
\newcommand{\atW}{a_{\PQt\,\scriptscriptstyle{\PW}}}
\newcommand{\auW}{a_{\PQu\,\scriptscriptstyle{\PW}}}
\newcommand{\atB}{a_{\PQt\,\scriptscriptstyle{\PB}}}
\newcommand{\auB}{a_{\PQu\,\scriptscriptstyle{\PB}}}
\newcommand{\afWB}{a_{\Pf\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\auWB}{a_{\PQu\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\auBW}{a_{\PQu\,\scriptscriptstyle{\PB\PW}}}
\newcommand{\atWB}{a_{\PQt\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\atBW}{a_{\PQt\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\aUW}{a_{\sPQU\,\scriptscriptstyle{\PW}}}
\newcommand{\aUB}{a_{\sPQU\,\scriptscriptstyle{\PB}}}
\newcommand{\aUWB}{a_{\sPQU\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\aUBW}{a_{\sPQU\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\abW}{a_{\PQb\,\scriptscriptstyle{\PW}}}
\newcommand{\adW}{a_{\PQd\,\scriptscriptstyle{\PW}}}
\newcommand{\abB}{a_{\PQb\,\scriptscriptstyle{\PB}}}
\newcommand{\adB}{a_{\PQd\,\scriptscriptstyle{\PB}}}
\newcommand{\adWB}{a_{\PQd\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\adBW}{a_{\PQd\,\scriptscriptstyle{\PB\PW}}}
\newcommand{\abWB}{a_{\PQb\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\abBW}{a_{\PQb\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\aDW}{a_{\sPQD\,\scriptscriptstyle{\PW}}}
\newcommand{\aDB}{a_{\sPQD\,\scriptscriptstyle{\PB}}}
\newcommand{\aDWB}{a_{\sPQD\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\aDBW}{a_{\sPQD\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\alW}{a_{\Pl\,\scriptscriptstyle{\PW}}}
\newcommand{\alB}{a_{\Pl\,\scriptscriptstyle{\PB}}}
\newcommand{\alWB}{a_{\Pl\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\alBW}{a_{\Pl\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\aLW}{a_{\sPL\,\scriptscriptstyle{\PW}}}
\newcommand{\aLB}{a_{\sPL\,\scriptscriptstyle{\PB}}}
\newcommand{\aLWB}{a_{\sPL\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\aLBW}{a_{\sPL\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\aplWt}{a^{(3)}_{\upphi\,\Pl\,\scriptscriptstyle{\PW}}}
\newcommand{\apqWt}{a^{(3)}_{\upphi\,\PQq\,\scriptscriptstyle{\PW}}}
\newcommand{\apQWt}{a^{(3)}_{\upphi\,\sPQQ\,\scriptscriptstyle{\PW}}}
%
\newcommand{\aplV}{a_{\upphi\,\Pl\,\scriptscriptstyle{\PV}}}
\newcommand{\aplA}{a_{\upphi\,\Pl\,\scriptscriptstyle{\PA}}}
\newcommand{\apfV}{a_{\upphi\,\Pf\,\scriptscriptstyle{\PV}}}
\newcommand{\apuV}{a_{\upphi\,\PQu\,\scriptscriptstyle{\PV}}}
\newcommand{\aptV}{a_{\upphi\,\PQt\,\scriptscriptstyle{\PV}}}
\newcommand{\apfA}{a_{\upphi\,\Pf\,\scriptscriptstyle{\PA}}}
\newcommand{\apuA}{a_{\upphi\,\PQu\,\scriptscriptstyle{\PA}}}
\newcommand{\aptA}{a_{\upphi\,\PQt\,\scriptscriptstyle{\PA}}}
\newcommand{\apUV}{a_{\upphi\,\sPQU\,\scriptscriptstyle{\PV}}}
\newcommand{\apUA}{a_{\upphi\,\sPQU\,\scriptscriptstyle{\PA}}}
\newcommand{\apdV}{a_{\upphi\,\PQd\,\scriptscriptstyle{\PV}}}
\newcommand{\apbV}{a_{\upphi\,\PQb\,\scriptscriptstyle{\PV}}}
\newcommand{\apdA}{a_{\upphi\,\PQd\,\scriptscriptstyle{\PA}}}
\newcommand{\apbA}{a_{\upphi\,\PQb\,\scriptscriptstyle{\PA}}}
\newcommand{\apDV}{a_{\upphi\,\sPQD\,\scriptscriptstyle{\PV}}}
\newcommand{\apDA}{a_{\upphi\,\sPQD\,\scriptscriptstyle{\PA}}}
\newcommand{\apn}{a_{\upphi\,\PGn}}
%
\newcommand{\aplo}{a^{(1)}_{\upphi\,\Pl}}
\newcommand{\aplt}{a^{(3)}_{\upphi\,\Pl}}
\newcommand{\apqo}{a^{(1)}_{\upphi\,\PQq}}
\newcommand{\apQo}{a^{(1)}_{\upphi\,\sPQQ}}
\newcommand{\apqt}{a^{(3)}_{\upphi\,\PQq}}
%
\newcommand{\apLo}{a^{(1)}_{\upphi\,\sPL}}
\newcommand{\apLt}{a^{(3)}_{\upphi\,\sPL}}
\newcommand{\apQt}{a^{(3)}_{\upphi\,\sPQQ}}
%
\newcommand{\apq}{a_{\upphi\,\PQq}}
\newcommand{\apu}{a_{\upphi\,\PQu}}
\newcommand{\apd}{a_{\upphi\,\PQd}}
\newcommand{\apl}{a_{\upphi\,\Pl}}
%
\newcommand{\apQ}{a_{\upphi\,\sPQQ}}
\newcommand{\apU}{a_{\upphi\,\sPQU}}
\newcommand{\apDq}{a_{\upphi\,\sPQD}}
\newcommand{\apL}{a_{\upphi\,\sPL}}
%
\newcommand{\aLldQ}{a_{\sPL\,\Pl\,\PQd\,\sPQQ}}
\newcommand{\aoQuQd}{a^{(1)}_{\sPQQ\,\PQu\,\sPQQ\,\PQd}}
\newcommand{\aoLlQu}{a^{(1)}_{\sPL\,\Pl\,\sPQQ\,\PQu}}
%
\newcommand{\bfun}[3]{\mrB_0^{\fin}\lpar #1\,;\,#2\,,\,#3\rpar}
\newcommand{\sbfun}[2]{\mrB_0^{\fin}\lpar #1\,,\,#2\rpar}
\newcommand{\bfunp}[3]{\mrB_{0\mathrm{p}}^{\fin}\lpar #1\,;\,#2\,,\,#3\rpar}
\newcommand{\bfuns}[3]{\mrB_{0\mathrm{s}}^{\fin}\lpar #1\,;\,#2\,,\,#3\rpar}
%
\newcommand{\zbfunp}[2]{\mrB_{0\mathrm{p}}^{\fin}\lpar \,#1\,,\,#2\rpar}
\newcommand{\zbfuns}[2]{\mrB_{0\mathrm{s}}^{\fin}\lpar \,#1\,,\,#2\rpar}
%
\newcommand{\ssp}{\mathrm{p}}
%
\newcommand{\WC}[1]{\ssW_{#1}}
\newcommand{\WCr}[1]{\ssW^{\ren}_{#1}}
%
\newcommand{\vtqs}{\mathrm{v}^2_{\PQt}}
\newcommand{\vbqs}{\mathrm{v}^2_{\PQb}}
\newcommand{\vtq}{\mathrm{v}_{\PQt}}
\newcommand{\vbq}{\mathrm{v}_{\PQb}}
%
\newcommand{\vqu}{\mathrm{v}_{\PQu}}
\newcommand{\vqd}{\mathrm{v}_{\PQd}}
\newcommand{\vle}{\mathrm{v}_{\Pl}}
\newcommand{\vqus}{\mathrm{v}^2_{\PQu}}
\newcommand{\vqds}{\mathrm{v}^2_{\PQd}}
\newcommand{\vles}{\mathrm{v}^2_{\Pl}}
%
\newcommand{\vple}{\mathrm{v}^{+}_{\Pl}}
\newcommand{\vpqu}{\mathrm{v}^{+}_{\PQu}}
\newcommand{\vpqd}{\mathrm{v}^{+}_{\PQd}}
\newcommand{\vmle}{\mathrm{v}^{-}_{\Pl}}
\newcommand{\vmqu}{\mathrm{v}^{-}_{\PQu}}
\newcommand{\vmqd}{\mathrm{v}^{-}_{\PQd}}
%
%\newcommand{\sla}[1]{/\!\!\!#1}
\newcommand{\sla}[1]{/\!\!\!\!\!#1}
%
\newcommand{\OPI}{1\mathrm{PI}}
\newcommand{\OPR}{1\mathrm{PR}}
%
\newcommand{\IR}{1\mathrm{IR}}
%
\newcommand{\DUV}{\Delta_{\mathrm{UV}}}
\newcommand{\DIR}{\Delta_{\mathrm{IR}}}
\newcommand{\LUV}{{\mathrm L}_{\mathrm{UV}}}
\newcommand{\DUVM}{\Delta_{\mathrm{UV}}\lpar \mws \rpar}
%
\newcommand{\cfun}[6]{\ssC_0\lpar #1\,,\,#2\,,\,#3\,;\,#4\,,\,#5\,,\,#6\rpar}
\newcommand{\cfunf}[6]{\ssC^{\fin}_0\lpar #1\,,\,#2\,,\,#3\,;\,#4\,,\,#5\,,\,#6\rpar}
\newcommand{\scfun}[2]{\ssC_0\lpar #1\,;\,#2\rpar}
%
%\newcommand{\sbfun}[2]{b^{\fin}_0\lpar #1\,,\,#2 \rpar}
\newcommand{\afun}[1]{a^{\fin}_0\lpar #1 \rpar}
%
\newcommand{\hyp}[4]{{}_2\,\mrF_1\lpar #1\,,\,#2\,;\,#3\,;\,#4\rpar}
%
\newcommand{\xptvi}{x^6_{\PQt}}
\newcommand{\xpbvi}{x^6_{\PQb}}
%
\newcommand{\xphvi}{x^6_{\sPH}}
\newcommand{\xphq}{x^4_{\sPH}}
\newcommand{\xpuq}{x^4_{\PQu}}
\newcommand{\xptq}{x^4_{\PQt}}
\newcommand{\xpdq}{x^4_{\PQd}}
\newcommand{\xpbq}{x^4_{\PQb}}
\newcommand{\xplq}{x^4_{\Pl}}
%
\newcommand{\xpss}{x^2_{\sPS}}
\newcommand{\xphs}{x^2_{\sPH}}
\newcommand{\xpus}{x^2_{\PQu}}
\newcommand{\xpts}{x^2_{\PQt}}
\newcommand{\xpds}{x^2_{\PQd}}
\newcommand{\xpbs}{x^2_{\PQb}}
\newcommand{\xpls}{x^2_{\Pl}}
\newcommand{\xpuc}{x^3_{\PQu}}
\newcommand{\xpdc}{x^3_{\PQd}}
\newcommand{\xplc}{x^3_{\Pl}}
%
\newcommand{\xpUs}{x^2_{\sPQU}}
\newcommand{\xpDs}{x^2_{\sPQD}}
\newcommand{\xpLs}{x^2_{\sPL}}
%--
\newcommand{\xps}{x_{\sPS}}
\newcommand{\xph}{x_{\sPH}}
\newcommand{\xpu}{x_{\PQu}}
\newcommand{\xpd}{x_{\PQd}}
\newcommand{\xpl}{x_{\Pl}}
%
\DeclareRobustCommand{\xog}{x^{(1)}_{\gen}}
\DeclareRobustCommand{\xtg}{x^{(2)}_{\gen}}
\DeclareRobustCommand{\vog}{v^{(1)}_{\gen}}
\DeclareRobustCommand{\vtg}{v^{(2)}_{\gen}}
%--
%
\newcommand{\sumg}{\sum_{\ggen}}
%
\newcommand{\xpUq}{x^4_{\sPQU}}
\newcommand{\xpDq}{x^4_{\sPQD}}
\newcommand{\xpLq}{x^4_{\sPL}}
\newcommand{\xpLc}{x^3_{\sPL}}
\newcommand{\xpUc}{x^3_{\sPQU}}
\newcommand{\xpDc}{x^3_{\sPQD}}
%
\newcommand{\xpU}{x_{\sPQU}}
\newcommand{\xpD}{x_{\sPQD}}
\newcommand{\xpL}{x_{\sPL}}
%
\newcommand{\vpus}{\mathrm{v}^2_{\PQu}}
\newcommand{\vpds}{\mathrm{v}^2_{\PQd}}
\newcommand{\vpls}{\mathrm{v}^2_{\Pl}}
%
\newcommand{\vpu}{\mathrm{v}_{\PQu}}
\newcommand{\vpd}{\mathrm{v}_{\PQd}}
\newcommand{\vpl}{\mathrm{v}_{\Pl}}
%
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\mcE}{\mathcal{E}}
%--
\newcommand{\mcO}{\mathcal{O}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcS}{\mathcal{S}}
\newcommand{\mcH}{\mathcal{H}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcW}{\mathcal{W}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcY}{\mathcal{Y}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\mcZ}{\mathcal{Z}}
%
\newcommand{\myNG}{{\mathrm N}_{\gen}}
\newcommand{\LR}{{\mathrm L}_{\ssR}}
\newcommand{\Lir}{{\mathrm L}_{\mathrm{ir}}}
\newcommand{\mrdim}{\mathrm{dim}}
\newcommand{\cdim}{\mathrm{codim}}
%
\newcommand{\UVsl}{{\mathrm C}^{\sPL}_{\mathrm{UV}}}
\newcommand{\UVst}{{\mathrm C}^{\sPQU}_{\mathrm{UV}}}
\newcommand{\UVsb}{{\mathrm C}^{\sPQD}_{\mathrm{UV}}}
%
\newcommand{\lzs}{\lambda^2_{\sPZ}}
\newcommand{\lz}{\lambda_{\sPZ}}
\newcommand{\lws}{\lambda^2_{\sPW}}
\newcommand{\lw}{\lambda_{\sPW}}
%
\newcommand{\lazs}{\lambda^2_{\sPA\sPZ}}
\newcommand{\lzzs}{\lambda^2_{\sPZ\sPZ}}
\newcommand{\lwws}{\lambda^2_{\sPW\sPW}}
%
\newcommand{\laz}{\lambda_{\sPA\sPZ}}
\newcommand{\lzz}{\lambda_{\sPZ\sPZ}}
\newcommand{\lww}{\lambda_{\sPW\sPW}}
%
\newcommand{\WFHs}{\mrW^{(6)}_{\PH}}
\newcommand{\WFWs}{\mrW^{(6)}_{\PW}}
\newcommand{\degfs}{\mathrm{d}\mcZ^{(6)}_g}
\newcommand{\dMfs}{\mathrm{d}\mcZ^{(6)}_{\mw}}
%
\newcommand{\WFH}{\mrW^{(4)}_{\PH}}
\newcommand{\WFA}{\mrW^{(4)}_{\PA}}
\newcommand{\WFZ}{\mrW^{(4)}_{\PZ}}
\newcommand{\WFW}{\mrW^{(4)}_{\PW}}
\newcommand{\degf}{\mathrm{d}\mcZ^{(4)}_g}
\newcommand{\dMf}{\mathrm{d}\mcZ^{(4)}_{\mw}}
\newcommand{\dcthf}{\mathrm{d}\mcZ^{(4)}_c}
%
\newcommand{\WFZt}{\mrW^{(4)}_{\PZ\,\mid\,\PQt}}
\newcommand{\WFZb}{\mrW^{(4)}_{\PZ\,\mid\,\PQb}}
\newcommand{\WFZW}{\mrW^{(4)}_{\PZ\,\mid\,\PW}}
\newcommand{\WFZrf}{{\overline{\sum}}_{\gen}\,\mrW^{(4)}_{\PZ\,\mid\,\Pf}}
%
\newcommand{\WFHt}{\mrW^{(4)}_{\PH\,\mid\,\PQt}}
\newcommand{\WFHb}{\mrW^{(4)}_{\PH\,\mid\,\PQb}}
\newcommand{\WFHW}{\mrW^{(4)}_{\PH\,\mid\,\PW}}
\newcommand{\WFHtb}{\mrW^{(4)}_{\PH\,\mid\,\PQt,\PQb}}
%
\newcommand{\dMff}{\sum_{\gen}\,\mathrm{d}\mcZ^{(4)}_{M\,\mid\,\Pf}}
\newcommand{\dMfW}{\mathrm{d}\mcZ^{(4)}_{M\,\mid\,\PW}}
\newcommand{\dMftb}{\mathrm{d}\mcZ^{(4)}_{M\,\mid\,\PQt,\PQb}}
\newcommand{\dMfrf}{{\overline{\sum}}_{\gen}\,\mathrm{d}\mcZ^{(4)}_{M\,\mid\,\Pf}}
%
\newcommand{\degfrf}{\sum_{\gen}\,\mathrm{d}\mcZ^{(4)}_{g\,\mid\,\Pf}}
\newcommand{\degfW}{\mathrm{d}\mcZ^{(4)}_{g\,\mid\,\PW}}
\newcommand{\degftb}{\mathrm{d}\mcZ^{(4)}_{g\,\mid\,\PQt,\PQb}}
\newcommand{\degff}{\sum_{\gen}\,\mathrm{d}\mcZ^{(4)}_{g\,\mid\,\Pf}}
%
\newcommand{\dcthft}{\mathrm{d}\mcZ^{(4)}_{\ctw\,\mid\,\PQt}}
\newcommand{\dcthfb}{\mathrm{d}\mcZ^{(4)}_{\ctw\,\mid\,\PQb}}
\newcommand{\dcthfrf}{{\overline{\sum}}_{\gen}\,\mathrm{d}\mcZ^{(4)}_{\ctw\,\mid\,\Pf}}
\newcommand{\dcthfW}{\mathrm{d}\mcZ^{(4)}_{\ctw\,\mid\,\PW}}
%
\newcommand{\WFWtb}{\mrW^{(4)}_{\PW\,\mid\,\PQt,\PQb}}
\newcommand{\WFWW}{\mrW^{(4)}_{\PW\,\mid\,\PW}}
\newcommand{\WFWrf}{{\overline{\sum}}_{\gen}\,\mrW^{(4)}_{\PW\,\mid\,\Pf}}
%
\newcommand{\Dg}{\Delta g}
%
\newcommand{\spc}{\,,}
\newcommand{\spp}{\,\,.}
%
\newcommand{\gds}{g_{_6}}
%
\newcommand{\blueref}[1]{{\color{NavyBlue}{#1}}}
\newcommand{\redeq}[1]{{\color{BrickRed}{#1}}}
%
\newcommand{\proA}[1]{\Delta_{\sPA}(#1)}
\newcommand{\proZ}[1]{\Delta_{\sPZ}(#1)}
%
\newcommand{\DR}{\mathrm{DR}}
\newcommand{\SR}{\mathrm{SR}}
\newcommand{\NR}{\mathrm{NR}}
%
\newcommand{\sPAZ}{{\scriptscriptstyle{\PA\PZ}}}
\newcommand{\bmidl}{\Bigr|\Xspace}
\newcommand{\bmidr}{\Xspace\Bigr|}
\newcommand{\proZb}[1]{{\overline{\Delta}}_{\sPZ}(#1)}
\newcommand{\muV}{\mathswitch{\mu_{\sPV}}}
\newcommand{\muVs}{\mathswitch{\mu^2_{\sPV}}}
\newcommand{\gamV}{\mathswitch{\gamma_{\sPV}}}
\newcommand{\gamVs}{\mathswitch{\gamma^2_{\sPV}}}
\newcommand{\reg}{{\mbox{\scriptsize reg}}}
%
\newcommand{\muZ}{\mathswitch{\mu_{\sPZ}}}
\newcommand{\muZs}{\mathswitch{\mu^2_{\sPZ}}}
\newcommand{\gamZ}{\mathswitch{\gamma_{\sPZ}}}
\newcommand{\gamZs}{\mathswitch{\gamma^2_{\sPZ}}}
%
\newcommand{\PO}{\mathrm{\scriptscriptstyle{PO}}}
%
\newcommand{\egam}[1]{\Gamma(#1)}
%
\DeclareRobustCommand{\PWpL}{\HepParticle{\PW}{\PL}{+}\Xspace}
\DeclareRobustCommand{\PWmL}{\HepParticle{\PW}{\PL}{-}\Xspace}
%
\DeclareRobustCommand{\PAe}{\HepAntiParticle{\Pe}{}{}\Xspace}
%--
\newcommand{\tcif}{\mathswitch {I^{(3)}_{\Pf}}}
%
\newcommand{\sft}{{\mbox{\scriptsize soft}}}
%
\newcommand{\gsix}{\mathswitch {g_{_6}}}
%
\newcommand{\gve}{{{g^{\Pe}_{\sPV}}}}
\newcommand{\gae}{{{g^{\Pe}_{\sPA}}}}
\newcommand{\gvf}{{{g^{\Pf}_{\sPV}}}}
\newcommand{\gaf}{{{g^{\Pf}_{\sPA}}}}
\newcommand{\Qe}{Q_{\Pe}}
\newcommand{\Qf}{Q_{\Pf}}
\newcommand{\Qes}{Q^2_{\Pe}}
\newcommand{\Qfs}{Q^2_{\Pf}}
%
\newcommand{\sone}{s_{_1}}
\newcommand{\stwo}{s_{_2}}
\newcommand{\sPAA}{{\scriptscriptstyle{\PA\PA}}}
\newcommand{\spinub}[1]{\mybar{{\mathrm{u}}}_{#1}}
\newcommand{\spinu}[1]{{\mathrm{u}}_{#1}}
\newcommand{\spinv}[1]{{\mathrm{v}}_{#1}}
\newcommand{\mcQ}{\mathcal{Q}}
\newcommand{\sPHZ}{{\scriptscriptstyle{\PH\PZ}}}
%
\newcommand{\spinubL}[1]{\mybar{{\mathrm{u}}}_{#1\,\scriptscriptstyle{\mrL}}}
\newcommand{\spinubR}[1]{\mybar{{\mathrm{u}}}_{#1\,\scriptscriptstyle{\mrR}}}
\newcommand{\spinvL}[1]{{\mathrm{v}}_{#1\,\scriptscriptstyle{\mrL}}}
\newcommand{\spinvR}[1]{{\mathrm{v}}_{#1\,\scriptscriptstyle{\mrR}}}
%
\newcommand{\sbe}{\sin\beta}
\newcommand{\cbe}{\cos\beta}
\newcommand{\sbes}{\sin^2\beta}
\newcommand{\cbes}{\cos^2\beta}
\newcommand{\sbeq}{\sin^4\beta}
\newcommand{\cbeq}{\cos^4\beta}
\newcommand{\tbe}{\tan\beta}
\newcommand{\tbes}{\tan^2\beta}
\newcommand{\stbe}{\sin(2\,\beta)}
\newcommand{\ctbe}{\cos(2\,\beta)}
\newcommand{\sab}{\sin(\alpha - \beta)}
\newcommand{\cab}{\cos(\alpha - \beta)}
\newcommand{\sabs}{\sin^2(\alpha - \beta)}
\newcommand{\cabs}{\cos^2(\alpha - \beta)}
%
\newcommand{\Msb}{{\overline M}}
\newcommand{\Msbs}{{\overline M}^2}
\newcommand{\lb}{{\overline \lambda}}
\newcommand{\tb}{{\overline t}}
\newcommand{\mrFb}{{\overline \mrF}}
%
\newcommand{\dbe}{\delta_{\beta}}
\newcommand{\dal}{\delta_{\alpha}}
%
\DeclareRobustCommand{\PHpm}{\HepParticle{\PH}{}{\,\pm}\Xspace}
\DeclareRobustCommand{\PAz}{\HepParticle{\PA}{}{\,0}\Xspace}
\DeclareRobustCommand{\PHp}{\HepParticle{\PH}{}{+}\Xspace}
\DeclareRobustCommand{\PHm}{\HepParticle{\PH}{}{-}\Xspace}
%
\DeclareRobustCommand{\PKz}{\HepParticle{\upPhi}{0}{2}\Xspace}
\DeclareRobustCommand{\PKh}{\HepParticle{\upPhi}{\Ph}{2}\Xspace}
%
\DeclareRobustCommand{\PKzs}{\HepParticle{\upPhi}{0}{4}\Xspace}
\DeclareRobustCommand{\PKhs}{\HepParticle{\upPhi}{\Ph}{4}\Xspace}
%
\DeclareRobustCommand{\PKzc}{\HepParticle{\upPhi}{0}{6}\Xspace}
\DeclareRobustCommand{\PKhc}{\HepParticle{\upPhi}{\Ph}{6}\Xspace}
%
\DeclareRobustCommand{\CDmu}{\HepParticle{\PD}{\mu}{}\Xspace}
\DeclareRobustCommand{\pdmu}{\HepParticle{\partial}{\mu}{}\Xspace}
\DeclareRobustCommand{\pdnu}{\HepParticle{\partial}{\nu}{}\Xspace}
%
%\DeclareRobustCommand{\PuPz}{\HepParticle{\upPhi}{0}{}\Xspace}
%\DeclareRobustCommand{\PuPh}{\HepParticle{\upPhi}{\Ph}{}\Xspace}
%\DeclareRobustCommand{\PuPzd}{\HepParticle{\upPhi}{0}{\dagger}\Xspace}
%\DeclareRobustCommand{\PuPhd}{\HepParticle{\upPhi}{\Ph}{\dagger}\Xspace}
%%
%\DeclareRobustCommand{\PKz}{\PuPzd\,\PuPz}
%\DeclareRobustCommand{\PKh}{\PuPhd\,\upPhi_{\Ph}}
%\DeclareRobustCommand{\PKzs}{\lpar \PuPzd\,\PuPz \rpar^2}
%\DeclareRobustCommand{\PKhs}{\lpar \PuPhd\,\PuPh \rpar^2}
%\DeclareRobustCommand{\PKzc}{\lpar \PuPzd\,\PuPz \rpar^3}
%\DeclareRobustCommand{\PKhc}{\lpar \PuPhd\,\PuPh \rpar^3}
%--
\newcommand{\pdmuPh}{\pdmu\,\Ph}
\newcommand{\pdmuPpz}{\pdmu\,\Ppz}
\newcommand{\pdmuPpp}{\pdmu\,\Ppp}
\newcommand{\pdmuPpm}{\pdmu\,\Ppm}
\newcommand{\pdmuPKh}{\pdmu\,\PKh}
\newcommand{\pdmuPKhs}{\pdmu\,\PKh\,\pdmu\,\PKh}
\newcommand{\PkinA}{\pdmu\,\PAdnu\,\pdmu\,\PAdnu}
\newcommand{\PkinZ}{\pdmu\,\PZdnu\,\pdmu\,\PZdnu}
\newcommand{\PkinW}{\pdmu\,\PWpdnu\,\pdmu\,\PWmdnu}
\newcommand{\PDQu}{\CDmu\,\PQu}
\newcommand{\PDQd}{\CDmu\,\PQd}
\newcommand{\PdivA}{\pdmu\,\PAdmu}
\newcommand{\PdivZ}{\pdmu\,\PZdmu}
\newcommand{\PdivWp}{\pdmu\,\PWpdmu}
\newcommand{\PdivWm}{\pdmu\,\PWmdmu}
\newcommand{\PWpnumu}{\pdnu\,\PWpdmu}
\newcommand{\PWmnumu}{\pdnu\,\PWmdmu}
\newcommand{\PdAnumu}{\pdnu\,\PAdmu}
\newcommand{\PdZnumu}{\pdnu\,\PZdmu}
\newcommand{\PdXmmu}{\pdmu\,\PXm}
\newcommand{\PdXpmu}{\pdmu\,\PXp}
\newcommand{\PdYamu}{\pdmu\,\PYa}
\newcommand{\PdYzmu}{\pdmu\,\PYz}
\newcommand{\PZdmus}{\PZdmu\,\PZdmu}
\newcommand{\PdmuPpp}{\CDmu\,\Ppp}
\newcommand{\PdmuPpm}{\CDmu\,\Ppm}
\newcommand{\PdmuPppm}{\CDmu\,\Ppp\,\CDmu\,\Ppm}
\newcommand{\PdAXmmu}{\pdmu\,\PAXm}
\newcommand{\PdAXpmu}{\pdmu\,\PAXp}
\newcommand{\PdAYamu}{\pdmu\,\PAYa}
\newcommand{\PdAYzmu}{\pdmu\,\PAYz}
\newcommand{\PdWpnumu}{\pdnu\,\PWpmu}
\newcommand{\PdWmnumu}{\pdnu\,\PWmmu}
%
\newcommand{\MSB}{{\overline{\mathrm{MS}}}}
%
\newcommand{\Nf}{\mathbb{N}}
\newcommand{\Rf}{\mathbb{R}}
\newcommand{\Cf}{\mathbb{C}}
\newcommand{\dsimp}[1]{\int\,dS_{#1}}
\newcommand{\dcub}[1]{\int\,dC_{#1}}
\newcommand{\dsimpd}{\int\,dS^d_2}
\newcommand{\dcubs}[2]{\int\,dCS\lpar #1\,;\,#2 \rpar}
\newcommand{\pd}{\scriptscriptstyle{+}}
\newcommand{\ppd}{\scriptscriptstyle{++}}
\newcommand{\pppd}{\scriptscriptstyle{+++}}
\newcommand{\mrLi}{{\mathrm{Li}}}
\newcommand{\tHs}{\mu_{\mathrm{DR}}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

